Measurement of the branching fraction and $\it CP$-violating asymmetry of the decay $B^{0} \rightarrow \pi^{0} \pi^{0}$ using $387$ million bottom-antibottom meson pairs in Belle II data

We measure the branching fraction and $\it CP$-violating flavor-dependent rate asymmetry of $B^{0} \to \pi^{0} \pi^{0}$ decays reconstructed using the Belle II detector in an electron-positron collision sample containing $387 \times 10^{6}$ $B\overline{B}$ pairs. Using an optimized event selection, we find $126\pm 20$ signal decays in a fit to background-discriminating and flavor-sensitive distributions. The resulting branching fraction is $(1.25 \pm 0.23)\times 10^{-6}$ and the $\it CP$-violating asymmetry is $0.03 \pm 0.30$.

==> authors-PRIVATE.tex <==
%%% Paper:    B0 to pi0 pi0
%%% Journal:  Physical Review D Letter
%%% Contacts:  S. Raiz, M. Dorigo, D. Tonelli
%%% ====================================================================
%%% Use \input{pub057} to insert this material into your latex file.
\newcommand{\instKAU}{Department of Physics, Faculty of Science, King Abdulaziz University, Jeddah 21589, Saudi Arabia}
\newcommand{\instSinica}{Academia Sinica, Taipei 11529, Taiwan}
\newcommand{\instCPPM}{Aix Marseille Universit\'{e}, CNRS/IN2P3, CPPM, 13288 Marseille, France}
\newcommand{\instYerevan}{Alikhanyan National Science Laboratory, Yerevan 0036, Armenia}
\newcommand{\instGoettingen}{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen, Germany}
\newcommand{\instBeihang}{Beihang University, Beijing 100191, China}
\newcommand{\instBNL}{Brookhaven National Laboratory, Upton, New York 11973, U.S.A.}
\newcommand{\instBINP}{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090, Russian Federation}
\newcommand{\instCMU}{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, U.S.A.}
\newcommand{\instCinvestavIPN}{Centro de Investigacion y de Estudios Avanzados del Instituto Politecnico Nacional, Mexico City 07360, Mexico}
\newcommand{\instPrague}{Faculty of Mathematics and Physics, Charles University, 121 16 Prague, Czech Republic}
\newcommand{\instChiangMai}{Chiang Mai University, Chiang Mai 50202, Thailand}
\newcommand{\instChiba}{Chiba University, Chiba 263-8522, Japan}
\newcommand{\instChonnam}{Chonnam National University, Gwangju 61186, South Korea}
\newcommand{\instChula}{Chulalongkorn University, Bangkok 10330, Thailand}
\newcommand{\instCAU}{Chung-Ang University, Seoul 06974, South Korea}
\newcommand{\instConacyt}{Consejo Nacional de Ciencia y Tecnolog\'{\i}a, Mexico City 03940, Mexico}
\newcommand{\instDESY}{Deutsches Elektronen--Synchrotron, 22607 Hamburg, Germany}
\newcommand{\instDuke}{Duke University, Durham, North Carolina 27708, U.S.A.}
\newcommand{\instITAR}{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000, Vietnam}
\newcommand{\instFuJen}{Department of Physics, Fu Jen Catholic University, Taipei 24205, Taiwan}
\newcommand{\instFudan}{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, China}
\newcommand{\instGifu}{Gifu University, Gifu 501-1193, Japan}
\newcommand{\instSOKENDAI}{The Graduate University for Advanced Studies (Sokendai), Tsukuba 305-0801, Japan}
\newcommand{\instMainz}{Institut f\"{u}r Kernphysik, Johannes Gutenberg-Universit\"{a}t Mainz, D-55099 Mainz, Germany}
\newcommand{\instGyeongsang}{Gyeongsang National University, Jinju 52828, South Korea}
\newcommand{\instHanyang}{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763, South Korea}
\newcommand{\instHeidelberg}{Heidelberg University, 68131 Mannheim, Germany}
\newcommand{\instHNU}{Henan Normal University, Xinxiang 453007, China}
\newcommand{\instKEK}{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\newcommand{\instJPARC}{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\newcommand{\instHiroshima}{Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8530, Japan}
\newcommand{\instHUNNU}{Hunan Normal University, Changsha 410081, China}
\newcommand{\instFrascati}{INFN Laboratori Nazionali di Frascati, I-00044 Frascati, Italy}
\newcommand{\instNapoliINFN}{INFN Sezione di Napoli, I-80126 Napoli, Italy}
\newcommand{\instPadovaINFN}{INFN Sezione di Padova, I-35131 Padova, Italy}
\newcommand{\instPerugiaINFN}{INFN Sezione di Perugia, I-06123 Perugia, Italy}
\newcommand{\instPisaINFN}{INFN Sezione di Pisa, I-56127 Pisa, Italy}
\newcommand{\instRomaTreINFN}{INFN Sezione di Roma Tre, I-00146 Roma, Italy}
\newcommand{\instTorinoINFN}{INFN Sezione di Torino, I-10125 Torino, Italy}
\newcommand{\instTriesteINFN}{INFN Sezione di Trieste, I-34127 Trieste, Italy}
\newcommand{\instIISc}{Indian Institute of Science, Bengaluru 560012, India}
\newcommand{\instIISER}{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306, India}
\newcommand{\instIITBhubaneswar}{Indian Institute of Technology Bhubaneswar, Bhubaneswar 752050, India}
\newcommand{\instIITGuwahati}{Indian Institute of Technology Guwahati, Assam 781039, India}
\newcommand{\instIITHyderabad}{Indian Institute of Technology Hyderabad, Telangana 502285, India}
\newcommand{\instIITJodhpur}{Indian Institute of Technology Jodhpur, Jodhpur 342030, India}
\newcommand{\instIITMadras}{Indian Institute of Technology Madras, Chennai 600036, India}
\newcommand{\instIndiana}{Indiana University, Bloomington, Indiana 47408, U.S.A.}
\newcommand{\instIHEPRussia}{Institute for High Energy Physics, Protvino 142281, Russian Federation}
\newcommand{\instHEPHYVienna}{Institute of High Energy Physics, Vienna 1050, Austria}
\newcommand{\instIHEPChina}{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
\newcommand{\instIPP}{Institute of Particle Physics (Canada), Victoria, British Columbia V8W 2Y2, Canada}
\newcommand{\instIOP}{Institute of Physics, Vietnam Academy of Science and Technology (VAST), Hanoi, Vietnam}
\newcommand{\instIFIC}{Instituto de Fisica Corpuscular, Paterna 46980, Spain}
\newcommand{\instISU}{Iowa State University, Ames, Iowa 50011, U.S.A.}
\newcommand{\instJAEA}{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195, Japan}
\newcommand{\instJLU}{Jilin University, Changchun 130012, China}
\newcommand{\instKarlsruhe}{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe, Germany}
\newcommand{\instKitasato}{Kitasato University, Sagamihara 252-0373, Japan}
\newcommand{\instKISTI}{Korea Institute of Science and Technology Information, Daejeon 34141, South Korea}
\newcommand{\instKoreaUnivKU}{Korea University, Seoul 02841, South Korea}
\newcommand{\instKSU}{Kyoto Sangyo University, Kyoto 603-8555, Japan}
\newcommand{\instKyotoU}{Kyoto University, Kyoto 606-8501, Japan}
\newcommand{\instKyungpook}{Kyungpook National University, Daegu 41566, South Korea}
\newcommand{\instLNNU}{Liaoning Normal University, Dalian 116029, China}
\newcommand{\instGiessen}{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en, Germany}
\newcommand{\instLuther}{Luther College, Decorah, Iowa 52101, U.S.A.}
\newcommand{\instMNITJaipur}{Malaviya National Institute of Technology Jaipur, Jaipur 302017, India}
\newcommand{\instLMU}{Ludwig Maximilians University, 80539 Munich, Germany}
\newcommand{\instMcGill}{McGill University, Montr\'{e}al, Qu\'{e}bec, H3A 2T8, Canada}
\newcommand{\instMETU}{Middle East Technical University, 06531 Ankara, Turkey}
\newcommand{\instMEPhI}{Moscow Physical Engineering Institute, Moscow 115409, Russian Federation}
\newcommand{\instNagoya}{Graduate School of Science, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNagoyaIAR}{Institute for Advanced Research, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNagoyaKMI}{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNNU}{Nanjing Normal University, Nanjing 210023, China}
\newcommand{\instNankai}{Nankai University, Tianjin 300071, China}
\newcommand{\instNaraWu}{Nara Women's University, Nara 630-8506, Japan}
\newcommand{\instUNAM}{National Autonomous University of Mexico, Mexico City, Mexico}
\newcommand{\instHSE}{National Research University Higher School of Economics, Moscow 101000, Russian Federation}
\newcommand{\instNTUTaiwan}{Department of Physics, National Taiwan University, Taipei 10617, Taiwan}
\newcommand{\instNUUTaiwan}{National United University, Miao Li 36003, Taiwan}
\newcommand{\instKrakow}{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342, Poland}
\newcommand{\instNiigata}{Niigata University, Niigata 950-2181, Japan}
\newcommand{\instNSU}{Novosibirsk State University, Novosibirsk 630090, Russian Federation}
\newcommand{\instOsakaMetropolitan}{Osaka Metropolitan University, Osaka 558-8585, Japan}
\newcommand{\instRCNP}{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047, Japan}
\newcommand{\instPNNL}{Pacific Northwest National Laboratory, Richland, Washington 99352, U.S.A.}
\newcommand{\instPanjab}{Panjab University, Chandigarh 160014, India}
\newcommand{\instPeking}{Peking University, Beijing 100871, China}
\newcommand{\instMPP}{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen, Germany}
\newcommand{\instMPGHLL}{Semiconductor Laboratory of the Max Planck Society, 81739 M\"{u}nchen, Germany}
\newcommand{\instPanjabPAU}{Punjab Agricultural University, Ludhiana 141004, India}
\newcommand{\instRIKENMSL}{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198, Japan}
\newcommand{\instSeoul}{Seoul National University, Seoul 08826, South Korea}
\newcommand{\instShandong}{Shandong University, Jinan 250100, China}
\newcommand{\instKyiv}{Taras Shevchenko National University of Kiev, Kiev, Ukraine}
\newcommand{\instSPU}{Showa Pharmaceutical University, Tokyo 194-8543, Japan}
\newcommand{\instSoochow}{Soochow University, Suzhou 215006, China}
\newcommand{\instSoongsil}{Department of Physics and Origin of Matter and Evolution of Galaxy (OMEG) Institute, Soongsil University, Seoul 06978, South Korea}
\newcommand{\instSEU}{Southeast University, Nanjing 211189, China}
\newcommand{\instLjubljanaJSI}{J. Stefan Institute, 1000 Ljubljana, Slovenia}
\newcommand{\instSKKU}{Sungkyunkwan University, Suwon 16419, South Korea}
\newcommand{\instTata}{Tata Institute of Fundamental Research, Mumbai 400005, India}
\newcommand{\instTUM}{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
\newcommand{\instTelAviv}{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978, Israel}
\newcommand{\instToho}{Toho University, Funabashi 274-8510, Japan}
\newcommand{\instTohoku}{Department of Physics, Tohoku University, Sendai 980-8578, Japan}
\newcommand{\instTitech}{Tokyo Institute of Technology, Tokyo 152-8550, Japan}
\newcommand{\instTokyoMetropolitan}{Tokyo Metropolitan University, Tokyo 192-0397, Japan}
\newcommand{\instUAS}{Universidad Autonoma de Sinaloa, Sinaloa 80000, Mexico}
\newcommand{\instNapoliUNIV}{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli, Italy}
\newcommand{\instPadovaUNIV}{Dipartimento di Fisica e Astronomia, Universit\`{a} di Padova, I-35131 Padova, Italy}
\newcommand{\instPerugiaUNIV}{Dipartimento di Fisica, Universit\`{a} di Perugia, I-06123 Perugia, Italy}
\newcommand{\instPisaUNIV}{Dipartimento di Fisica, Universit\`{a} di Pisa, I-56127 Pisa, Italy}
\newcommand{\instRomaTreUNIV}{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma, Italy}
\newcommand{\instTorinoUNIV}{Dipartimento di Fisica, Universit\`{a} di Torino, I-10125 Torino, Italy}
\newcommand{\instTriesteUNIV}{Dipartimento di Fisica, Universit\`{a} di Trieste, I-34127 Trieste, Italy}
\newcommand{\instMontreal}{Universit\'{e} de Montr\'{e}al, Physique des Particules, Montr\'{e}al, Qu\'{e}bec, H3C 3J7, Canada}
\newcommand{\instIJCLab}{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\newcommand{\instIPHC}{Universit\'{e} de Strasbourg, CNRS, IPHC, UMR 7178, 67037 Strasbourg, France}
\newcommand{\instAdelaide}{Department of Physics, University of Adelaide, Adelaide, South Australia 5005, Australia}
\newcommand{\instUofA}{University of Alberta, Edmonton, Alberta, T6G 2E1, Canada}
\newcommand{\instBonn}{University of Bonn, 53115 Bonn, Germany}
\newcommand{\instUBC}{University of British Columbia, Vancouver, British Columbia, V6T 1Z1, Canada}
\newcommand{\instCincinnati}{University of Cincinnati, Cincinnati, Ohio 45221, U.S.A.}
\newcommand{\instFlorida}{University of Florida, Gainesville, Florida 32611, U.S.A.}
\newcommand{\instHamburg}{University of Hamburg, 20148 Hamburg, Germany}
\newcommand{\instHawaii}{University of Hawaii, Honolulu, Hawaii 96822, U.S.A.}
\newcommand{\instLjubljanaUniLJ}{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana, Slovenia}
\newcommand{\instLouisville}{University of Louisville, Louisville, Kentucky 40292, U.S.A.}
\newcommand{\instMalaya}{National Centre for Particle Physics, University of Malaya, 50603 Kuala Lumpur, Malaysia}
\newcommand{\instManitoba}{University of Manitoba, Winnipeg, Manitoba, R3T 2N2, Canada}
\newcommand{\instLjubljanaUM}{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor, Slovenia}
\newcommand{\instMelbourne}{School of Physics, University of Melbourne, Victoria 3010, Australia}
\newcommand{\instMississippi}{University of Mississippi, University, Mississippi 38677, U.S.A.}
\newcommand{\instUOM}{University of Miyazaki, Miyazaki 889-2192, Japan}
\newcommand{\instNovaGorica}{University of Nova Gorica, 5000 Nova Gorica, Slovenia}
\newcommand{\instUPES}{University of Petroleum and Energy Studies, Dehradun 248007, India}
\newcommand{\instPittsburgh}{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, U.S.A.}
\newcommand{\instUSTC}{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026, China}
\newcommand{\instSAlabama}{University of South Alabama, Mobile, Alabama 36688, U.S.A.}
\newcommand{\instSCarolina}{University of South Carolina, Columbia, South Carolina 29208, U.S.A.}
\newcommand{\instSydney}{School of Physics, University of Sydney, New South Wales 2006, Australia}
\newcommand{\instTabuk}{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451, Saudi Arabia}
\newcommand{\instUTokyo}{Department of Physics, University of Tokyo, Tokyo 113-0033, Japan}
\newcommand{\instEri}{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032, Japan}
\newcommand{\instIPMU}{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583, Japan}
\newcommand{\instVictoria}{University of Victoria, Victoria, British Columbia, V8W 3P6, Canada}
\newcommand{\instUppsala}{Uppsala University, SE-751 05 Uppsala, Sweden}
\newcommand{\instVPI}{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, U.S.A.}
\newcommand{\instWayneState}{Wayne State University, Detroit, Michigan 48202, U.S.A.}
\newcommand{\instXavier}{St. Francis Xavier University, Antigonish, Nova Scotia, B2G 2W5, Canada}
\newcommand{\instXJTU}{Xi'an Jiaotong University, Xi'an 710049, China}
\newcommand{\instYamagata}{Yamagata University, Yamagata 990-8560, Japan}
\newcommand{\instYonsei}{Yonsei University, Seoul 03722, South Korea}
\newcommand{\instTYL}{Toshiko Yuasa Laboratory, Tsukuba 305-0801, Japan}
\newcommand{\instZZU}{Zhengzhou University, Zhengzhou 450001, China}
%%%\affiliation{\instKAU}
%%%\affiliation{\instSinica}
\affiliation{\instCPPM}
\affiliation{\instYerevan}
\affiliation{\instGoettingen}
%%%\affiliation{\instBeihang}
\affiliation{\instBNL}
\affiliation{\instBINP}
\affiliation{\instCMU}
\affiliation{\instCinvestavIPN}
\affiliation{\instPrague}
\affiliation{\instChiangMai}
\affiliation{\instChiba}
\affiliation{\instChonnam}
\affiliation{\instChula}
\affiliation{\instCAU}
\affiliation{\instConacyt}
\affiliation{\instDESY}
\affiliation{\instDuke}
\affiliation{\instITAR}
\affiliation{\instFuJen}
\affiliation{\instFudan}
\affiliation{\instGifu}
\affiliation{\instSOKENDAI}
\affiliation{\instMainz}
\affiliation{\instGyeongsang}
\affiliation{\instHanyang}
\affiliation{\instHeidelberg}
\affiliation{\instHNU}
\affiliation{\instKEK}
\affiliation{\instJPARC}
\affiliation{\instHiroshima}
\affiliation{\instHUNNU}
\affiliation{\instFrascati}
\affiliation{\instNapoliINFN}
\affiliation{\instPadovaINFN}
\affiliation{\instPerugiaINFN}
\affiliation{\instPisaINFN}
\affiliation{\instRomaTreINFN}
\affiliation{\instTorinoINFN}
\affiliation{\instTriesteINFN}
\affiliation{\instIISc}
\affiliation{\instIISER}
\affiliation{\instIITBhubaneswar}
\affiliation{\instIITGuwahati}
\affiliation{\instIITHyderabad}
\affiliation{\instIITJodhpur}
\affiliation{\instIITMadras}
\affiliation{\instIndiana}
\affiliation{\instIHEPRussia}
\affiliation{\instHEPHYVienna}
\affiliation{\instIHEPChina}
\affiliation{\instIPP}
\affiliation{\instIOP}
\affiliation{\instIFIC}
\affiliation{\instISU}
\affiliation{\instJAEA}
\affiliation{\instJLU}
\affiliation{\instKarlsruhe}
\affiliation{\instKitasato}
\affiliation{\instKISTI}
\affiliation{\instKoreaUnivKU}
\affiliation{\instKSU}
\affiliation{\instKyotoU}
\affiliation{\instKyungpook}
\affiliation{\instLNNU}
\affiliation{\instGiessen}
\affiliation{\instLuther}
\affiliation{\instMNITJaipur}
\affiliation{\instLMU}
\affiliation{\instMcGill}
%%%\affiliation{\instMETU}
%%%\affiliation{\instMEPhI}
\affiliation{\instNagoya}
%%%\affiliation{\instNagoyaIAR}
\affiliation{\instNagoyaKMI}
%%%\affiliation{\instNNU}
\affiliation{\instNankai}
\affiliation{\instNaraWu}
%%%\affiliation{\instUNAM}
\affiliation{\instHSE}
\affiliation{\instNTUTaiwan}
\affiliation{\instNUUTaiwan}
\affiliation{\instKrakow}
\affiliation{\instNiigata}
\affiliation{\instNSU}
\affiliation{\instOsakaMetropolitan}
\affiliation{\instRCNP}
\affiliation{\instPNNL}
\affiliation{\instPanjab}
%%%\affiliation{\instPeking}
\affiliation{\instMPP}
\affiliation{\instMPGHLL}
\affiliation{\instPanjabPAU}
\affiliation{\instRIKENMSL}
%%%\affiliation{\instSeoul}
\affiliation{\instShandong}
\affiliation{\instKyiv}
\affiliation{\instSPU}
\affiliation{\instSoochow}
\affiliation{\instSoongsil}
\affiliation{\instSEU}
\affiliation{\instLjubljanaJSI}
\affiliation{\instSKKU}
\affiliation{\instTata}
\affiliation{\instTUM}
\affiliation{\instTelAviv}
\affiliation{\instToho}
%%%\affiliation{\instTohoku}
\affiliation{\instTitech}
\affiliation{\instTokyoMetropolitan}
\affiliation{\instUAS}
\affiliation{\instNapoliUNIV}
\affiliation{\instPadovaUNIV}
\affiliation{\instPerugiaUNIV}
\affiliation{\instPisaUNIV}
\affiliation{\instRomaTreUNIV}
\affiliation{\instTorinoUNIV}
\affiliation{\instTriesteUNIV}
%%%\affiliation{\instMontreal}
\affiliation{\instIJCLab}
\affiliation{\instIPHC}
\affiliation{\instAdelaide}
\affiliation{\instUofA>
\affiliation{\instBonn}
\affiliation{\instUBC}
\affiliation{\instCincinnati}
\affiliation{\instFlorida}
\affiliation{\instHamburg}
\affiliation{\instHawaii}
\affiliation{\instLjubljanaUniLJ}
\affiliation{\instLouisville}
\affiliation{\instMalaya}
\affiliation{\instManitoba}
\affiliation{\instLjubljanaUM}
\affiliation{\instMelbourne}
\affiliation{\instMississippi}
\affiliation{\instUOM}
\affiliation{\instNovaGorica}
\affiliation{\instUPES}
\affiliation{\instPittsburgh}
\affiliation{\instUSTC}
\affiliation{\instSAlabama}
\affiliation{\instSCarolina}
\affiliation{\instSydney}
\affiliation{\instTabuk}
\affiliation{\instUTokyo}
\affiliation{\instEri}
\affiliation{\instIPMU}
\affiliation{\instVictoria}
\affiliation{\instUppsala}
\affiliation{\instVPI}
\affiliation{\instWayneState}
\affiliation{\instXavier}
\affiliation{\instXJTU}
\affiliation{\instYamagata}
\affiliation{\instYonsei}
\affiliation{\instTYL}
%%%\affiliation{\instZZU}
  \author{I.~Adachi}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2590
% \author{K.~Adamczyk}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2239
  \author{L.~Aggarwal}\affiliation{\instPanjab} % 10083
% \author{P.~Ahlburg}\affiliation{\instBonn} % 2367
  \author{H.~Ahmed}\affiliation{\instXavier} % 11323
% \author{J.~K.~Ahn}\affiliation{\instKoreaUnivKU} % 7423
  \author{H.~Aihara}\affiliation{\instUTokyo} % 2223
% \author{N.~Akopov}\affiliation{\instYerevan} % 9443
  \author{M.~Alhakami}\affiliation{\instTabuk} % 28103
  \author{A.~Aloisio}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2194
  \author{N.~Althubiti}\affiliation{\instTabuk} % 21524
% \author{L.~Andricek}\affiliation{\instMPGHLL} % 2098
% \author{M.~Angelsmark}\affiliation{\instBonn} % 13963
  \author{N.~Anh~Ky}\affiliation{\instIOP} % 2218
  \author{D.~M.~Asner}\affiliation{\instBNL} % 4684
  \author{H.~Atmacan}\affiliation{\instCincinnati} % 2538
% \author{V.~Aulchenko}\affiliation{\instBINP}\affiliation{\instNSU} % 8183
% \author{T.~Aushev}\affiliation{\instHSE} % 3747
  \author{V.~Aushev}\affiliation{\instKyiv} % 2155
  \author{M.~Aversano}\affiliation{\instNagoya} % 7363
  \author{R.~Ayad}\affiliation{\instTabuk} % 3766
% \author{T.~Aziz}\affiliation{\instTata} % 3523
  \author{V.~Babu}\affiliation{\instIPHC} % 5623
% \author{S.~Bacher}\affiliation{\instKrakow} % 2258
  \author{H.~Bae}\affiliation{\instKEK} % 10863
  \author{N.~K.~Baghel}\affiliation{\instLouisville} % 21505
  \author{S.~Bahinipati}\affiliation{\instIITBhubaneswar} % 2332
% \author{A.~M.~Bakich}\affiliation{\instSydney} % 2115
  \author{P.~Bambade}\affiliation{\instIJCLab} % 3003
  \author{Sw.~Banerjee}\affiliation{\instLouisville} % 8603
  \author{S.~Bansal}\affiliation{\instPanjab} % 5163
  \author{M.~Barrett}\affiliation{\instKEK} % 2180
  \author{M.~Bartl}\affiliation{\instMPP} % 26483
% \author{G.~Batignani}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 6643
  \author{J.~Baudot}\affiliation{\instIPHC} % 2562
% \author{M.~Bauer}\affiliation{\instKarlsruhe} % 9863
  \author{A.~Baur}\affiliation{\instDESY} % 5683
  \author{A.~Beaubien}\affiliation{\instVictoria} % 6683
  \author{F.~Becherer}\affiliation{\instDESY} % 21623
  \author{J.~Becker}\affiliation{\instKarlsruhe} % 5403
% \author{P.~K.~Behera}\affiliation{\instIITMadras} % 4204
  \author{J.~V.~Bennett}\affiliation{\instMississippi} % 2454
% \author{E.~Bernieri}\affiliation{\instRomaTreINFN} % 4483
  \author{F.~U.~Bernlochner}\affiliation{\instBonn} % 2282
  \author{V.~Bertacchi}\affiliation{\instCPPM} % 2212
  \author{M.~Bertemes}\affiliation{\instHEPHYVienna} % 2595
  \author{E.~Bertholet}\affiliation{\instTelAviv} % 13163
  \author{M.~Bessner}\affiliation{\instHawaii} % 3783
  \author{S.~Bettarini}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2350
  \author{V.~Bhardwaj}\affiliation{\instIISER} % 2228
  \author{B.~Bhuyan}\affiliation{\instIITGuwahati} % 2097
  \author{F.~Bianchi}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2564
% \author{L.~Bierwirth}\affiliation{\instTUM} % 11723
  \author{T.~Bilka}\affiliation{\instDESY} % 2484
% \author{S.~Bilokin}\affiliation{\instLMU} % 3623
  \author{D.~Biswas}\affiliation{\instLouisville} % 8703
% \author{T.~Bloomfield}\affiliation{\instKEK} % 2418
  \author{A.~Bobrov}\affiliation{\instBINP}\affiliation{\instNSU} % 2294
  \author{D.~Bodrov}\affiliation{\instSoochow}\affiliation{\instHSE} % 9643
  \author{A.~Bolz}\affiliation{\instDESY} % 15403
  \author{A.~Bondar}\affiliation{\instBINP}\affiliation{\instNSU} % 4643
% \author{G.~Bonvicini}\affiliation{\instWayneState} % 2095
  \author{J.~Borah}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 7083
  \author{A.~Boschetti}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 17683
  \author{A.~Bozek}\affiliation{\instKrakow} % 2303
  \author{M.~Bra\v{c}ko}\affiliation{\instLjubljanaJSI}\affiliation{\instLjubljanaUM} % 2425
  \author{P.~Branchini}\affiliation{\instRomaTreINFN} % 2577
% \author{N.~Brenny}\affiliation{\instISU} % 19943
  \author{R.~A.~Briere}\affiliation{\instCMU} % 2584
  \author{T.~E.~Browder}\affiliation{\instHawaii} % 2560
% \author{Y.~Buch}\affiliation{\instGoettingen} % 17323
  \author{A.~Budano}\affiliation{\instRomaTreINFN} % 2171
  \author{S.~Bussino}\affiliation{\instRomaTreUNIV}\affiliation{\instRomaTreINFN} % 5384
% \author{A.~Calcaterra}\affiliation{\instFrascati} % 19163
  \author{Q.~Campagna}\affiliation{\instMississippi} % 21563
  \author{M.~Campajola}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 5223
  \author{L.~Cao}\affiliation{\instDESY} % 2099
  \author{G.~Casarosa}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2491
  \author{C.~Cecchi}\affiliation{\instPerugiaUNIV}\affiliation{\instPerugiaINFN} % 2433
  \author{J.~Cerasoli}\affiliation{\instIPHC} % 20746
  \author{M.-C.~Chang}\affiliation{\instFuJen} % 2827
  \author{P.~Chang}\affiliation{\instNTUTaiwan} % 2542
  \author{R.~Cheaib}\affiliation{\instDESY} % 2208
  \author{P.~Cheema}\affiliation{\instSydney} % 15264
% \author{V.~Chekelian}\affiliation{\instMPP} % 2167
% \author{C.~Chen}\affiliation{\instISU} % 12803
% \author{Y.~Q.~Chen}\affiliation{\instJLU} % 16264
% \author{Y.-T.~Chen}\affiliation{\instNTUTaiwan} % 2884
  \author{B.~G.~Cheon}\affiliation{\instHanyang} % 2173
  \author{K.~Chilikin}\affiliation{\instBINP} % 2308
  \author{K.~Chirapatpimol}\affiliation{\instChiangMai} % 10803
  \author{H.-E.~Cho}\affiliation{\instHanyang} % 2182
  \author{K.~Cho}\affiliation{\instKISTI} % 2516
  \author{S.-J.~Cho}\affiliation{\instYonsei} % 2723
  \author{S.-K.~Choi}\affiliation{\instCAU} % 2364
  \author{S.~Choudhury}\affiliation{\instISU} % 2206
% \author{K.~Chu}\affiliation{\instMcGill} % 5203
% \author{D.~Cinabro}\affiliation{\instWayneState} % 2092
  \author{J.~Cochran}\affiliation{\instISU} % 12604
  \author{L.~Corona}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 3944
% \author{L.~M.~Cremaldi}\affiliation{\instMississippi} % 2276
  \author{J.~X.~Cui}\affiliation{\instSEU} % 8863
% \author{T.~Czank}\affiliation{\instTokyoMetropolitan} % 2254
% \author{S.~Das}\affiliation{\instMNITJaipur} % 9163
% \author{F.~Dattola}\affiliation{\instDESY} % 3745
  \author{E.~De~La~Cruz-Burelo}\affiliation{\instCinvestavIPN} % 2359
  \author{S.~A.~De~La~Motte}\affiliation{\instAdelaide} % 2128
  \author{G.~de~Marino}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 8364
  \author{G.~De~Nardo}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2459
% \author{M.~De~Nuccio}\affiliation{\instUBC} % 2610
  \author{G.~De~Pietro}\affiliation{\instKarlsruhe} % 2528
  \author{R.~de~Sangro}\affiliation{\instFrascati} % 2524
% \author{B.~Deschamps}\affiliation{\instBonn} % 2671
  \author{M.~Destefanis}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2594
  \author{S.~Dey}\affiliation{\instKEK} % 5023
% \author{A.~De~Yta-Hernandez}\affiliation{\instCinvestavIPN} % 2104
  \author{R.~Dhamija}\affiliation{\instIITHyderabad} % 9465
  \author{A.~Di~Canto}\affiliation{\instBNL} % 10963
  \author{F.~Di~Capua}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2065
  \author{J.~Dingfelder}\affiliation{\instBonn} % 2151
  \author{Z.~Dole\v{z}al}\affiliation{\instPrague} % 2319
  \author{I.~Dom\'{\i}nguez~Jim\'{e}nez}\affiliation{\instUAS} % 2191
  \author{T.~V.~Dong}\affiliation{\instITAR} % 2215
  \author{X.~Dong}\affiliation{\instDESY} % 17343
  \author{M.~Dorigo}\affiliation{\instTriesteINFN} % 12543
% \author{D.~Dorner}\affiliation{\instHEPHYVienna} % 13564
% \author{K.~Dort}\affiliation{\instGiessen} % 5583
  \author{D.~Dossett}\affiliation{\instMelbourne} % 2574
% \author{S.~Dreyer}\affiliation{\instDESY} % 12823
  \author{S.~Dubey}\affiliation{\instHawaii} % 11063
% \author{S.~Duell}\affiliation{\instBonn} % 2344
  \author{K.~Dugic}\affiliation{\instTUM} % 11103
  \author{G.~Dujany}\affiliation{\instIPHC} % 9703
  \author{P.~Ecker}\affiliation{\instKarlsruhe} % 5563
% \author{M.~Eliachevitch}\affiliation{\instBonn} % 2725
  \author{D.~Epifanov}\affiliation{\instBINP}\affiliation{\instNSU} % 2551
  \author{J.~Eppelt}\affiliation{\instKarlsruhe} % 19723
% \author{Y.~Fan}\affiliation{\instDESY} % 21303
  \author{P.~Feichtinger}\affiliation{\instHEPHYVienna} % 9843
  \author{T.~Ferber}\affiliation{\instKarlsruhe} % 2482
% \author{D.~Ferlewicz}\affiliation{\instMelbourne} % 2073
  \author{T.~Fillinger}\affiliation{\instKEK} % 9803
  \author{C.~Finck}\affiliation{\instIPHC} % 15803
  \author{G.~Finocchiaro}\affiliation{\instFrascati} % 2400
% \author{P.~Fischer}\affiliation{\instHeidelberg} % 2141
% \author{K.~Flood}\affiliation{\instHawaii} % 12103
  \author{A.~Fodor}\affiliation{\instMcGill} % 2312
  \author{F.~Forti}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2432
  \author{A.~Frey}\affiliation{\instGoettingen} % 2150
% \author{M.~Friedl}\affiliation{\instHEPHYVienna} % 2442
  \author{B.~G.~Fulsom}\affiliation{\instPNNL} % 2563
  \author{A.~Gabrielli}\affiliation{\instPisaINFN} % 13523
% \author{N.~Gabyshev}\affiliation{\instBINP}\affiliation{\instNSU} % 2510
  \author{E.~Ganiev}\affiliation{\instDESY} % 4623
  \author{M.~Garcia-Hernandez}\affiliation{\instKEK} % 4823
  \author{R.~Garg}\affiliation{\instCMU} % 2213
% \author{A.~Garmash}\affiliation{\instBINP}\affiliation{\instNSU} % 2161
  \author{G.~Gaudino}\affiliation{\instNapoliINFN} % 16563
  \author{V.~Gaur}\affiliation{\instUPES} % 2413
  \author{A.~Gaz}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 2181
% \author{U.~Gebauer}\affiliation{\instGoettingen} % 2174
  \author{A.~Gellrich}\affiliation{\instDESY} % 2480
  \author{G.~Ghevondyan}\affiliation{\instYerevan} % 9445
  \author{D.~Ghosh}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 11923
% \author{H.~Ghumaryan}\affiliation{\instYerevan} % 19543
  \author{G.~Giakoustidis}\affiliation{\instBonn} % 13723
  \author{R.~Giordano}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2103
  \author{A.~Giri}\affiliation{\instIITHyderabad} % 2106
  \author{P.~Gironella~Gironell}\affiliation{\instIPHC} % 25443
  \author{A.~Glazov}\affiliation{\instDESY} % 2473
  \author{B.~Gobbo}\affiliation{\instTriesteINFN} % 2109
  \author{R.~Godang}\affiliation{\instSAlabama} % 2449
  \author{O.~Gogota}\affiliation{\instKyiv} % 2334
  \author{P.~Goldenzweig}\affiliation{\instKarlsruhe} % 2345
% \author{B.~Golob}\affiliation{\instNovaGorica}\affiliation{\instLjubljanaJSI} % 3703
% \author{G.~Gong}\affiliation{\instUSTC} % 2727
% \author{P.~Grace}\affiliation{\instAdelaide} % 9563
  \author{W.~Gradl}\affiliation{\instMainz} % 2570
% \author{M.~Graf-Schreiber}\affiliation{\instDESY} % 2730
% \author{T.~Grammatico}\affiliation{\instVictoria} % 20623
  \author{S.~Granderath}\affiliation{\instBonn} % 8383
  \author{E.~Graziani}\affiliation{\instRomaTreINFN} % 2342
  \author{D.~Greenwald}\affiliation{\instTUM} % 2686
  \author{Z.~Gruberov\'{a}}\affiliation{\instPrague} % 8824
% \author{T.~Gu}\affiliation{\instPittsburgh} % 14283
  \author{Y.~Guan}\affiliation{\instCincinnati} % 2514
  \author{K.~Gudkova}\affiliation{\instBINP}\affiliation{\instNSU} % 10504
  \author{I.~Haide}\affiliation{\instKarlsruhe} % 14824
% \author{H.~Haigh}\affiliation{\instHEPHYVienna} % 16744
  \author{S.~Halder}\affiliation{\instTata} % 4743
  \author{Y.~Han}\affiliation{\instDESY} % 19663
% \author{K.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2462
  \author{T.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2523
  \author{C.~Harris}\affiliation{\instAdelaide} % 21383
% \author{O.~Hartbrich}\affiliation{\instHawaii} % 2158
  \author{K.~Hayasaka}\affiliation{\instNiigata} % 2330
  \author{H.~Hayashii}\affiliation{\instNaraWu} % 2455
  \author{S.~Hazra}\affiliation{\instMPP} % 7663
  \author{C.~Hearty}\affiliation{\instUBC}\affiliation{\instIPP} % 2450
  \author{M.~T.~Hedges}\affiliation{\instBonn} % 2265
  \author{A.~Heidelbach}\affiliation{\instKarlsruhe} % 16923
  \author{I.~Heredia~de~la~Cruz}\affiliation{\instCinvestavIPN}\affiliation{\instConacyt} % 2559
  \author{M.~Hern\'{a}ndez~Villanueva}\affiliation{\instBNL} % 2466
  \author{T.~Higuchi}\affiliation{\instIPMU} % 2485
% \author{H.~Hirata}\affiliation{\instNagoya} % 2070
  \author{M.~Hoek}\affiliation{\instMainz} % 2101
  \author{M.~Hohmann}\affiliation{\instMelbourne} % 2077
  \author{R.~Hoppe}\affiliation{\instDESY} % 23383
  \author{P.~Horak}\affiliation{\instHEPHYVienna} % 13583
% \author{T.~Hotta}\affiliation{\instRCNP} % 2084
  \author{C.-L.~Hsu}\affiliation{\instSydney} % 2299
% \author{A.~Huang}\affiliation{\instSydney} % 14223
% \author{K.~Huang}\affiliation{\instNTUTaiwan} % 2389
  \author{T.~Humair}\affiliation{\instDESY} % 10643
  \author{T.~Iijima}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI}\affiliation{\instKEK} % 2446
  \author{K.~Inami}\affiliation{\instNagoya}\affiliation{\instKEK} % 2323
% \author{G.~Inguglia}\affiliation{\instHEPHYVienna} % 2500
  \author{N.~Ipsita}\affiliation{\instIITHyderabad} % 12223
% \author{J.~Irakkathil~Jabbar}\affiliation{\instKarlsruhe} % 7343
  \author{A.~Ishikawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2281
% \author{S.~Ito}\affiliation{\instKEK} % 17463
  \author{R.~Itoh}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2487
  \author{M.~Iwasaki}\affiliation{\instOsakaMetropolitan} % 2360
% \author{Y.~Iwasaki}\affiliation{\instKEK} % 2229
% \author{S.~Iwata}\affiliation{\instTokyoMetropolitan} % 4323
  \author{P.~Jackson}\affiliation{\instAdelaide} % 2255
  \author{D.~Jacobi}\affiliation{\instBonn} % 15123
  \author{W.~W.~Jacobs}\affiliation{\instIndiana} % 2322
% \author{D.~E.~Jaffe}\affiliation{\instBNL} % 3663
  \author{E.-J.~Jang}\affiliation{\instGyeongsang} % 6744
  \author{Q.~P.~Ji}\affiliation{\instHNU} % 16243
  \author{S.~Jia}\affiliation{\instSEU} % 2457
  \author{Y.~Jin}\affiliation{\instBNL} % 2105
  \author{A.~Johnson}\affiliation{\instIITMadras} % 16143
  \author{K.~K.~Joo}\affiliation{\instChonnam} % 4224
  \author{H.~Junkerkalefeld}\affiliation{\instBonn} % 12963
% \author{I.~Kadenko}\affiliation{\instKyiv} % 3843
% \author{H.~Kakuno}\affiliation{\instTokyoMetropolitan} % 2391
% \author{M.~Kaleta}\affiliation{\instKrakow} % 5603
  \author{D.~Kalita}\affiliation{\instIITGuwahati} % 2220
  \author{A.~B.~Kaliyar}\affiliation{\instHEPHYVienna} % 7344
  \author{J.~Kandra}\affiliation{\instPadovaINFN} % 2541
  \author{K.~H.~Kang}\affiliation{\instIPMU} % 2283
  \author{S.~Kang}\affiliation{\instISU} % 12683
% \author{P.~Kapusta}\affiliation{\instKrakow} % 6663
  \author{G.~Karyan}\affiliation{\instYerevan} % 2550
% \author{Y.~Kato}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2549
% \author{H.~Kawai}\affiliation{\instChiba} % 4344
  \author{T.~Kawasaki}\affiliation{\instKitasato} % 4363
  \author{F.~Keil}\affiliation{\instMainz} % 19523
  \author{C.~Ketter}\affiliation{\instHawaii} % 2236
% \author{M.~Khan}\affiliation{\instBonn} % 15644
  \author{C.~Kiesling}\affiliation{\instMPP} % 2168
% \author{C.~Kim}\affiliation{\instYonsei} % 20503
  \author{C.-H.~Kim}\affiliation{\instHanyang} % 2358
  \author{D.~Y.~Kim}\affiliation{\instSoongsil} % 2315
% \author{H.~J.~Kim}\affiliation{\instKyungpook} % 4863
  \author{J.-Y.~Kim}\affiliation{\instYonsei} % 20223
  \author{K.-H.~Kim}\affiliation{\instKISTI} % 2118
% \author{K.~Kim}\affiliation{\instKoreaUnivKU} % 2409
  \author{Y.-K.~Kim}\affiliation{\instYonsei} % 2379
  \author{Y.~J.~Kim}\affiliation{\instKoreaUnivKU} % 2403
% \author{H.~Kindo}\affiliation{\instVPI}\affiliation{\instKEK} % 2195
  \author{K.~Kinoshita}\affiliation{\instCincinnati} % 2318
% \author{C.~Kleinwort}\affiliation{\instDESY} % 2499
  \author{P.~Kody\v{s}}\affiliation{\instPrague} % 2407
  \author{T.~Koga}\affiliation{\instKEK} % 6963
  \author{S.~Kohani}\affiliation{\instHawaii} % 9143
  \author{K.~Kojima}\affiliation{\instNagoya} % 6363
% \author{T.~Konno}\affiliation{\instKitasato} % 2490
% \author{H.~Korandla}\affiliation{\instHawaii} % 18783
  \author{A.~Korobov}\affiliation{\instBINP}\affiliation{\instNSU} % 4185
  \author{S.~Korpar}\affiliation{\instLjubljanaJSI}\affiliation{\instLjubljanaUM} % 2475
% \author{E.~Kou}\affiliation{\instIJCLab} % 3765
  \author{E.~Kovalenko}\affiliation{\instBINP}\affiliation{\instNSU} % 3884
  \author{R.~Kowalewski}\affiliation{\instVictoria} % 2293
% \author{T.~M.~G.~Kraetzschmar}\affiliation{\instMPP} % 7543
  \author{P.~Kri\v{z}an}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2474
% \author{R.~Kroeger}\affiliation{\instMississippi} % 2242
% \author{J.~F.~Krohn}\affiliation{\instMelbourne} % 2502
  \author{P.~Krokovny}\affiliation{\instBINP}\affiliation{\instNSU} % 2575
% \author{W.~Kuehn}\affiliation{\instGiessen} % 2534
% \author{M.~K\"{u}nzel}\affiliation{\instDESY}\affiliation{\instLMU} % 2139
  \author{T.~Kuhr}\affiliation{\instLMU} % 2486
  \author{Y.~Kulii}\affiliation{\instLMU} % 9823
  \author{D.~Kumar}\affiliation{\instIITGuwahati} % 7223
% \author{J.~Kumar}\affiliation{\instIITJodhpur} % 6464
  \author{M.~Kumar}\affiliation{\instIISER} % 2744
  \author{R.~Kumar}\affiliation{\instPanjabPAU} % 2189
  \author{K.~Kumara}\affiliation{\instMississippi} % 2257
% \author{T.~Kumita}\affiliation{\instTokyoMetropolitan} % 4083
  \author{T.~Kunigo}\affiliation{\instKEK} % 10104
% \author{A.~Kusudo}\affiliation{\instNaraWu} % 14623
  \author{A.~Kuzmin}\affiliation{\instBINP}\affiliation{\instNSU} % 2520
% \author{P.~Kvasni\v{c}ka}\affiliation{\instPrague} % 2184
  \author{Y.-J.~Kwon}\affiliation{\instYonsei} % 2231
  \author{S.~Lacaprara}\affiliation{\instPadovaINFN} % 2447
  \author{Y.-T.~Lai}\affiliation{\instKEK} % 2066
  \author{K.~Lalwani}\affiliation{\instMNITJaipur} % 2142
  \author{T.~Lam}\affiliation{\instVPI} % 2729
  \author{L.~Lanceri}\affiliation{\instTriesteINFN} % 2540
  \author{J.~S.~Lange}\affiliation{\instGiessen} % 2277
  \author{T.~S.~Lau}\affiliation{\instIJCLab} % 19803
  \author{M.~Laurenza}\affiliation{\instUppsala} % 10223
  \author{K.~Lautenbach}\affiliation{\instCPPM} % 2102
% \author{P.~J.~Laycock}\affiliation{\instBNL} % 7683
  \author{R.~Leboucher}\affiliation{\instUBC} % 14083
  \author{F.~R.~Le~Diberder}\affiliation{\instIJCLab} % 3267
  \author{M.~J.~Lee}\affiliation{\instSKKU} % 21803
% \author{S.~C.~Lee}\affiliation{\instKyungpook} % 2544
% \author{P.~Leitl}\affiliation{\instMPP} % 2414
  \author{C.~Lemettais}\affiliation{\instCPPM} % 22704
  \author{P.~Leo}\affiliation{\instDESY}\affiliation{\instHamburg} % 19823
  \author{D.~Levit}\affiliation{\instKEK} % 2507
  \author{P.~M.~Lewis}\affiliation{\instHawaii} % 2582
  \author{C.~Li}\affiliation{\instLNNU} % 2325
  \author{L.~K.~Li}\affiliation{\instCincinnati} % 3263
  \author{Q.~M.~Li}\affiliation{\instIHEPChina} % 22943
% \author{S.~X.~Li}\affiliation{\instFudan} % 2377
  \author{W.~Z.~Li}\affiliation{\instBeihang} % 19703
% \author{Y.~Li}\affiliation{\instFudan} % 8083
  \author{Y.~B.~Li}\affiliation{\instXJTU} % 2573
  \author{Y.~P.~Liao}\affiliation{\instIHEPChina} % 24303
  \author{J.~Libby}\affiliation{\instIITMadras} % 2262
% \author{K.~Lieret}\affiliation{\instLMU} % 2268
  \author{J.~Lin}\affiliation{\instNTUTaiwan} % 2401
  \author{S.~Lin}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 17223
% \author{Z.~Liptak}\affiliation{\instHiroshima} % 3565
% \author{A.~Little}\affiliation{\instSydney} % 23803
  \author{M.~H.~Liu}\affiliation{\instFudan} % 15244
  \author{Q.~Y.~Liu}\affiliation{\instHawaii} % 7045
  \author{Y.~Liu}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 16223
% \author{Z.~A.~Liu}\affiliation{\instIHEPChina} % 3283
  \author{Z.~Q.~Liu}\affiliation{\instShandong} % 11303
  \author{D.~Liventsev}\affiliation{\instWayneState}\affiliation{\instKEK} % 2578
  \author{S.~Longo}\affiliation{\instManitoba} % 2396
% \author{A.~Lozar}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 12423
  \author{T.~Lueck}\affiliation{\instLMU} % 2406
% \author{T.~Luo}\affiliation{\instFudan} % 3268
  \author{C.~Lyu}\affiliation{\instBonn} % 12484
  \author{Y.~Ma}\affiliation{\instRIKENMSL} % 16883
  \author{C.~Madaan}\affiliation{\instTata} % 25483
  \author{M.~Maggiora}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 5343
  \author{S.~P.~Maharana}\affiliation{\instIITHyderabad} % 19083
% \author{T.~Mahood}\affiliation{\instHawaii} % 26003
  \author{R.~Maiti}\affiliation{\instTorinoINFN} % 12043
  \author{S.~Maity}\affiliation{\instIITBhubaneswar} % 2985
  \author{G.~Mancinelli}\affiliation{\instCPPM} % 20743
  \author{R.~Manfredi}\affiliation{\instBNL} % 10303
  \author{E.~Manoni}\affiliation{\instPerugiaINFN} % 2305
% \author{A.~C.~Manthei}\affiliation{\instBonn} % 15023
  \author{M.~Mantovano}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 19783
  \author{D.~Marcantonio}\affiliation{\instMelbourne} % 11163
  \author{S.~Marcello}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 4223
  \author{C.~Marinas}\affiliation{\instIFIC} % 2133
% \author{L.~Martel}\affiliation{\instIPHC} % 13503
  \author{C.~Martellini}\affiliation{\instRomaTreINFN} % 16983
  \author{A.~Martens}\affiliation{\instIJCLab} % 13823
  \author{A.~Martini}\affiliation{\instDESY} % 2336
  \author{T.~Martinov}\affiliation{\instDESY} % 19463
  \author{L.~Massaccesi}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 16323
  \author{M.~Masuda}\affiliation{\instRCNP}\affiliation{\instEri} % 2238
  \author{T.~Matsuda}\affiliation{\instUOM} % 5543
% \author{K.~Matsuoka}\affiliation{\instKEK}\affiliation{\instNagoya} % 2316
  \author{D.~Matvienko}\affiliation{\instBINP}\affiliation{\instNSU} % 2351
  \author{S.~K.~Maurya}\affiliation{\instIITGuwahati} % 9763
  \author{M.~Maushart}\affiliation{\instIPHC} % 21203
% \author{F.~Mawas}\affiliation{\instIJCLab} % 20943
  \author{J.~A.~McKenna}\affiliation{\instUBC} % 2392
% \author{F.~Meggendorfer}\affiliation{\instMPP} % 7103
  \author{R.~Mehta}\affiliation{\instTata} % 15203
  \author{F.~Meier}\affiliation{\instDuke} % 3103
  \author{D.~Meleshko}\affiliation{\instGiessen} % 11523
  \author{M.~Merola}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2456
% \author{F.~Metzner}\affiliation{\instBonn} % 2296
% \author{M.~Milesi}\affiliation{\instMelbourne} % 5443
  \author{C.~Miller}\affiliation{\instVictoria} % 2273
  \author{M.~Mirra}\affiliation{\instNapoliINFN} % 14744
  \author{S.~Mitra}\affiliation{\instISU} % 19944
  \author{K.~Miyabayashi}\affiliation{\instNaraWu}\affiliation{\instKEK} % 2327
  \author{H.~Miyake}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2452
  \author{R.~Mizuk}\affiliation{\instIJCLab} % 2483
  \author{G.~B.~Mohanty}\affiliation{\instTata} % 2278
% \author{N.~Molina-Gonzalez}\affiliation{\instCinvestavIPN} % 8004
  \author{S.~Mondal}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 19743
  \author{S.~Moneta}\affiliation{\instPerugiaUNIV}\affiliation{\instPerugiaINFN} % 13303
% \author{H.~Moon}\affiliation{\instKoreaUnivKU} % 2304
  \author{H.-G.~Moser}\affiliation{\instMPP} % 2120
% \author{M.~Mrvar}\affiliation{\instHEPHYVienna} % 2527
% \author{Th.~Muller}\affiliation{\instKarlsruhe} % 2165
  \author{R.~Mussa}\affiliation{\instTorinoINFN} % 2372
  \author{I.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 3463
% \author{K.~R.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2417
% \author{E.~Nakano}\affiliation{\instOsakaMetropolitan} % 2554
  \author{M.~Nakao}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2498
% \author{H.~Nakayama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2232
% \author{H.~Nakazawa}\affiliation{\instNTUTaiwan} % 2335
  \author{Y.~Nakazawa}\affiliation{\instKEK}\affiliation{\instNagoyaKMI} % 17383
% \author{A.~Narimani~Charan}\affiliation{\instDESY} % 10143
  \author{M.~Naruki}\affiliation{\instKyotoU} % 4583
  \author{Z.~Natkaniec}\affiliation{\instKrakow} % 3923
  \author{A.~Natochii}\affiliation{\instBNL} % 12063
% \author{L.~Nayak}\affiliation{\instIITHyderabad} % 9464
  \author{M.~Nayak}\affiliation{\instIISc} % 2371
  \author{G.~Nazaryan}\affiliation{\instYerevan} % 9523
  \author{M.~Neu}\affiliation{\instKarlsruhe} % 23304
  \author{C.~Niebuhr}\affiliation{\instDESY} % 2477
% \author{M.~Niiyama}\affiliation{\instKSU} % 2063
% \author{J.~Ninkovic}\affiliation{\instMPGHLL} % 2386
% \author{N.~K.~Nisar}\affiliation{\instBNL} % 2522
  \author{S.~Nishida}\affiliation{\instKEK}\affiliation{\instSOKENDAI}\affiliation{\instNiigata} % 2571
% \author{K.~Nishimura}\affiliation{\instHawaii} % 3063
% \author{A.~Novosel}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 15523
% \author{K.~Ogawa}\affiliation{\instNiigata} % 2430
  \author{S.~Ogawa}\affiliation{\instToho} % 6263
% \author{R.~Okubo}\affiliation{\instNagoya} % 10743
% \author{S.~L.~Olsen}\affiliation{\instCAU} % 4563
% \author{Y.~Onishchuk}\affiliation{\instKyiv} % 2157
  \author{H.~Ono}\affiliation{\instNiigata} % 2160
  \author{Y.~Onuki}\affiliation{\instUTokyo} % 2331
% \author{P.~Oskin}\affiliation{\instIJCLab} % 9623
  \author{F.~Otani}\affiliation{\instUTokyo} % 16244
% \author{E.~R.~Oxford}\affiliation{\instCMU} % 6943
% \author{H.~Ozaki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2984
  \author{P.~Pakhlov}\affiliation{\instHSE} % 2221
  \author{G.~Pakhlova}\affiliation{\instHSE} % 2188
% \author{A.~Paladino}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2435
% \author{T.~Pang}\affiliation{\instPittsburgh} % 2114
% \author{A.~Panta}\affiliation{\instMississippi} % 7943
  \author{E.~Paoloni}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2488
  \author{S.~Pardi}\affiliation{\instNapoliINFN} % 2532
  \author{K.~Parham}\affiliation{\instDuke} % 10684
  \author{H.~Park}\affiliation{\instKyungpook} % 2284
  \author{J.~Park}\affiliation{\instUTokyo} % 18203
  \author{K.~Park}\affiliation{\instKISTI} % 12243
  \author{S.-H.~Park}\affiliation{\instKEK} % 2509
  \author{B.~Paschen}\affiliation{\instBonn} % 2159
  \author{A.~Passeri}\affiliation{\instRomaTreINFN} % 2116
  \author{S.~Patra}\affiliation{\instLouisville} % 3123
% \author{S.~Paul}\affiliation{\instTUM} % 2131
  \author{T.~K.~Pedlar}\affiliation{\instLuther} % 2421
  \author{I.~Peruzzi}\affiliation{\instFrascati} % 2253
  \author{R.~Peschke}\affiliation{\instHawaii} % 7123
  \author{R.~Pestotnik}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2476
% \author{F.~Pham}\affiliation{\instMelbourne} % 2963
  \author{M.~Piccolo}\affiliation{\instFrascati} % 2147
  \author{L.~E.~Piilonen}\affiliation{\instVPI} % 2346
% \author{G.~Pinna~Angioni}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 13363
  \author{P.~L.~M.~Podesta-Lerma}\affiliation{\instUAS} % 2266
  \author{T.~Podobnik}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 11223
  \author{S.~Pokharel}\affiliation{\instMississippi} % 12283
% \author{L.~Polat}\affiliation{\instCPPM} % 9783
% \author{V.~Popov}\affiliation{\instTelAviv}\affiliation{\instHSE} % 2096
  \author{C.~Praz}\affiliation{\instKEK} % 2726
  \author{S.~Prell}\affiliation{\instISU} % 12743
  \author{E.~Prencipe}\affiliation{\instGiessen} % 2219
  \author{M.~T.~Prim}\affiliation{\instBonn} % 2501
  \author{I.~Prudiiev}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 19383
% \author{M.~V.~Purohit}\affiliation{\instSCarolina} % 2196
  \author{H.~Purwar}\affiliation{\instHawaii} % 12363
% \author{N.~Rad}\affiliation{\instDESY} % 11683
  \author{P.~Rados}\affiliation{\instHEPHYVienna} % 7383
  \author{G.~Raeuber}\affiliation{\instHEPHYVienna} % 18143
  \author{S.~Raiz}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 13003
  \author{V.~RajG}\affiliation{\instIITMadras} % 24983
  \author{N.~Rauls}\affiliation{\instGoettingen} % 11603
  \author{K.~Ravindran}\affiliation{\instTata} % 22503
  \author{J.~U.~Rehman}\affiliation{\instKrakow} % 19623
  \author{M.~Reif}\affiliation{\instMPP} % 8043
  \author{S.~Reiter}\affiliation{\instGiessen} % 2248
  \author{M.~Remnev}\affiliation{\instBINP}\affiliation{\instNSU} % 2785
  \author{L.~Reuter}\affiliation{\instKarlsruhe} % 16403
  \author{D.~Ricalde~Herrmann}\affiliation{\instWayneState} % 9263
  \author{I.~Ripp-Baudot}\affiliation{\instIPHC} % 2469
% \author{M.~Ritzert}\affiliation{\instHeidelberg} % 2526
  \author{G.~Rizzo}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2579
% \author{L.~B.~Rizzuto}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 3746
% \author{S.~H.~Robertson}\affiliation{\instUofA}\affiliation{\instIPP} % 2471
% \author{P.~Rocchetti}\affiliation{\instMelbourne} % 13763
% \author{D.~Rodr\'{i}guez~P\'{e}rez}\affiliation{\instUAS} % 2176
  \author{M.~Roehrken}\affiliation{\instDESY} % 11883
  \author{J.~M.~Roney}\affiliation{\instVictoria}\affiliation{\instIPP} % 2244
% \author{C.~Rosenfeld}\affiliation{\instSCarolina} % 2082
  \author{A.~Rostomyan}\affiliation{\instDESY} % 2481
  \author{N.~Rout}\affiliation{\instTriesteINFN} % 2965
% \author{M.~Rozanska}\affiliation{\instKrakow} % 2205
% \author{G.~Russo}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2388
% \author{D.~Sahoo}\affiliation{\instISU} % 2110
% \author{Y.~Sakai}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2175
  \author{D.~A.~Sanders}\affiliation{\instMississippi} % 2458
  \author{S.~Sandilya}\affiliation{\instIITHyderabad} % 2286
% \author{A.~Sangal}\affiliation{\instCincinnati} % 2384
  \author{L.~Santelj}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2185
% \author{C.~Santos}\affiliation{\instIPHC} % 23743
% \author{P.~Sartori}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 4523
  \author{Y.~Sato}\affiliation{\instKEK} % 5243
  \author{V.~Savinov}\affiliation{\instPittsburgh} % 2292
  \author{B.~Scavino}\affiliation{\instUppsala} % 2518
  \author{C.~Schmitt}\affiliation{\instLMU}\affiliation{\instMPP} % 15063
% \author{J.~Schmitz}\affiliation{\instBonn} % 12863
  \author{S.~Schneider}\affiliation{\instDuke} % 16803
  \author{M.~Schnepf}\affiliation{\instKarlsruhe} % 15683
% \author{J.~Schueler}\affiliation{\instHawaii} % 2824
  \author{C.~Schwanda}\affiliation{\instHEPHYVienna} % 2108
  \author{A.~J.~Schwartz}\affiliation{\instCincinnati} % 2162
% \author{B.~Schwenker}\affiliation{\instGoettingen} % 2405
% \author{M.~Schwickardi}\affiliation{\instGoettingen} % 14743
  \author{Y.~Seino}\affiliation{\instNiigata} % 2517
  \author{A.~Selce}\affiliation{\instRomaTreINFN} % 9043
  \author{K.~Senyo}\affiliation{\instYamagata} % 2987
  \author{J.~Serrano}\affiliation{\instCPPM} % 12124
  \author{M.~E.~Sevior}\affiliation{\instMelbourne} % 2328
  \author{C.~Sfienti}\affiliation{\instMainz} % 2214
  \author{W.~Shan}\affiliation{\instHUNNU} % 11943
  \author{C.~Sharma}\affiliation{\instMNITJaipur} % 11584
% \author{G.~Sharma}\affiliation{\instIITMadras} % 18423
% \author{V.~Shebalin}\affiliation{\instHawaii} % 2339
  \author{C.~P.~Shen}\affiliation{\instFudan} % 2464
  \author{X.~D.~Shi}\affiliation{\instUTokyo} % 18843
% \author{H.~Shibuya}\affiliation{\instToho} % 2234
  \author{T.~Shillington}\affiliation{\instMcGill} % 7983
  \author{T.~Shimasaki}\affiliation{\instUTokyo} % 16263
  \author{J.-G.~Shiu}\affiliation{\instNTUTaiwan} % 2412
  \author{D.~Shtol}\affiliation{\instBINP}\affiliation{\instNSU} % 9223
% \author{B.~Shwartz}\affiliation{\instBINP}\affiliation{\instNSU} % 2122
  \author{A.~Sibidanov}\affiliation{\instHawaii} % 2419
  \author{F.~Simon}\affiliation{\instKarlsruhe} % 2164
  \author{J.~B.~Singh}\affiliation{\instPanjab}\affiliation{\instUPES} % 2903
  \author{J.~Skorupa}\affiliation{\instMPP}\affiliation{\instTUM} % 12523
% \author{K.~Smith}\affiliation{\instMelbourne} % 2243
  \author{R.~J.~Sobie}\affiliation{\instVictoria}\affiliation{\instIPP} % 2472
  \author{M.~Sobotzik}\affiliation{\instMainz} % 8604
  \author{A.~Soffer}\affiliation{\instTelAviv} % 2217
  \author{A.~Sokolov}\affiliation{\instIHEPRussia} % 2521
% \author{Y.~Soloviev}\affiliation{\instDESY} % 2479
  \author{E.~Solovieva}\affiliation{\instBINP} % 2398
  \author{W.~Song}\affiliation{\instJLU} % 22863
  \author{S.~Spataro}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2117
  \author{B.~Spruck}\affiliation{\instMainz} % 2493
  \author{M.~Stari\v{c}}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2326
  \author{P.~Stavroulakis}\affiliation{\instIPHC} % 20643
% \author{S.~Stefkova}\affiliation{\instKarlsruhe} % 8783
% \author{L.~Stoetzer}\affiliation{\instHawaii} % 19283
% \author{Z.~S.~Stottler}\affiliation{\instVPI} % 2267
  \author{R.~Stroili}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 2465
  \author{J.~Strube}\affiliation{\instPNNL} % 2451
  \author{Y.~Sue}\affiliation{\instNagoya} % 2085
% \author{R.~Sugiura}\affiliation{\instUTokyo} % 4644
  \author{M.~Sumihama}\affiliation{\instRCNP}\affiliation{\instGifu} % 4243
  \author{K.~Sumisawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI}\affiliation{\instNaraWu} % 2583
  \author{W.~Sutcliffe}\affiliation{\instBonn} % 3784
  \author{N.~Suwonjandee}\affiliation{\instChula} % 14063
% \author{S.~Y.~Suzuki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2496
  \author{H.~Svidras}\affiliation{\instDESY} % 11783
% \author{M.~Tabata}\affiliation{\instChiba} % 2986
  \author{M.~Takahashi}\affiliation{\instDESY} % 2467
  \author{M.~Takizawa}\affiliation{\instSPU}\affiliation{\instJPARC}\affiliation{\instRIKENMSL} % 2437
  \author{U.~Tamponi}\affiliation{\instTorinoINFN} % 2366
% \author{S.~Tanaka}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2530
  \author{K.~Tanida}\affiliation{\instJAEA} % 3803
% \author{H.~Tanigawa}\affiliation{\instUTokyo} % 2237
% \author{N.~Taniguchi}\affiliation{\instKEK} % 2285
  \author{F.~Tenchini}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2546
  \author{A.~Thaller}\affiliation{\instCPPM} % 16044
  \author{O.~Tittel}\affiliation{\instMPP} % 8663
  \author{R.~Tiwary}\affiliation{\instTata} % 10403
  \author{D.~Tonelli}\affiliation{\instTriesteINFN} % 4564
  \author{E.~Torassa}\affiliation{\instPadovaINFN} % 2556
% \author{N.~Toutounji}\affiliation{\instSydney} % 2263
  \author{K.~Trabelsi}\affiliation{\instTYL} % 2369
  \author{I.~Tsaklidis}\affiliation{\instBonn} % 13443
% \author{T.~Tsuboyama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2361
% \author{N.~Tsuzuki}\affiliation{\instNagoya} % 2352
  \author{M.~Uchida}\affiliation{\instTitech} % 2370
  \author{I.~Ueda}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2519
% \author{S.~Uehara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2586
% \author{Y.~Uematsu}\affiliation{\instUTokyo} % 5883
% \author{T.~Uglov}\affiliation{\instHSE} % 2252
  \author{K.~Unger}\affiliation{\instKarlsruhe} % 9463
  \author{Y.~Unno}\affiliation{\instHanyang} % 2420
  \author{K.~Uno}\affiliation{\instKEK} % 14963
  \author{S.~Uno}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2149
  \author{P.~Urquijo}\affiliation{\instMelbourne} % 2302
  \author{Y.~Ushiroda}\affiliation{\instKEK}\affiliation{\instUTokyo}\affiliation{\instSOKENDAI} % 2317
% \author{Y.~V.~Usov}\affiliation{\instBINP}\affiliation{\instNSU} % 5003
  \author{S.~E.~Vahsen}\affiliation{\instHawaii} % 2251
  \author{R.~van~Tonder}\affiliation{\instMcGill} % 2706
% \author{G.~S.~Varner}\affiliation{\instHawaii} % 2119
  \author{K.~E.~Varvell}\affiliation{\instSydney} % 2545
  \author{M.~Veronesi}\affiliation{\instISU} % 20723
% \author{A.~Vinokurova}\affiliation{\instBINP}\affiliation{\instNSU} % 2289
  \author{V.~S.~Vismaya}\affiliation{\instIITHyderabad} % 16063
  \author{L.~Vitale}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 2415
  \author{V.~Vobbilisetti}\affiliation{\instIFIC} % 7364
  \author{R.~Volpe}\affiliation{\instPerugiaUNIV}\affiliation{\instPerugiaINFN} % 20183
% \author{V.~Vorobyev}\affiliation{\instBINP} % 2298
  \author{A.~Vossen}\affiliation{\instDuke} % 2249
% \author{B.~Wach}\affiliation{\instMPP}\affiliation{\instTUM} % 8203
% \author{E.~Waheed}\affiliation{\instKEK} % 2226
  \author{M.~Wakai}\affiliation{\instUBC} % 3583
% \author{H.~M.~Wakeling}\affiliation{\instMcGill} % 3664
  \author{S.~Wallner}\affiliation{\instMPP} % 20363
% \author{W.~Wan~Abdullah}\affiliation{\instMalaya} % 2280
% \author{B.~Wang}\affiliation{\instCincinnati} % 2569
% \author{C.~H.~Wang}\affiliation{\instNUUTaiwan} % 2224
  \author{E.~Wang}\affiliation{\instPittsburgh} % 10983
  \author{M.-Z.~Wang}\affiliation{\instNTUTaiwan} % 2074
% \author{X.~L.~Wang}\affiliation{\instFudan} % 2076
  \author{Z.~Wang}\affiliation{\instUTokyo} % 15743
  \author{A.~Warburton}\affiliation{\instMcGill} % 2347
  \author{M.~Watanabe}\affiliation{\instNiigata} % 2309
  \author{S.~Watanuki}\affiliation{\instCincinnati} % 6843
% \author{M.~Welsch}\affiliation{\instBonn} % 7023
% \author{O.~Werbycka}\affiliation{\instTriesteINFN} % 6123
  \author{C.~Wessel}\affiliation{\instDESY} % 2100
% \author{J.~Wiechczynski}\affiliation{\instKrakow} % 2604
% \author{P.~Wieduwilt}\affiliation{\instGoettingen} % 2343
% \author{H.~Windel}\affiliation{\instMPP} % 2081
  \author{E.~Won}\affiliation{\instKoreaUnivKU} % 2410
% \author{Y.~Xie}\affiliation{\instShandong} % 20383
  \author{X.~P.~Xu}\affiliation{\instSoochow} % 4923
  \author{B.~D.~Yabsley}\affiliation{\instSydney} % 3645
  \author{S.~Yamada}\affiliation{\instKEK} % 2492
  \author{W.~Yan}\affiliation{\instUSTC} % 2094
  \author{S.~B.~Yang}\affiliation{\instKoreaUnivKU} % 2374
  \author{J.~Yelton}\affiliation{\instFlorida} % 2067
  \author{J.~H.~Yin}\affiliation{\instNankai} % 2365
% \author{Y.~M.~Yook}\affiliation{\instIHEPChina} % 2453
  \author{K.~Yoshihara}\affiliation{\instHawaii} % 12663
% \author{B.~Yu}\affiliation{\instLMU} % 15563
% \author{C.~Z.~Yuan}\affiliation{\instIHEPChina} % 2088
  \author{J.~Yuan}\affiliation{\instJLU} % 23423
% \author{Y.~Yusa}\affiliation{\instNiigata} % 2357
  \author{L.~Zani}\affiliation{\instRomaTreUNIV}\affiliation{\instRomaTreINFN} % 2529
  \author{F.~Zeng}\affiliation{\instIPMU} % 22043
  \author{B.~Zhang}\affiliation{\instHawaii} % 11663
% \author{J.~Z.~Zhang}\affiliation{\instIHEPChina} % 2349
% \author{Y.~Zhang}\affiliation{\instFudan} % 3303
% \author{Z.~Zhang}\affiliation{\instUSTC} % 5363
  \author{V.~Zhilich}\affiliation{\instBINP}\affiliation{\instNSU} % 4703
  \author{J.~S.~Zhou}\affiliation{\instFudan} % 12463
  \author{Q.~D.~Zhou}\affiliation{\instShandong} % 7323
% \author{X.~Y.~Zhou}\affiliation{\instLNNU} % 2380
% \author{L.~Zhu}\affiliation{\instJLU} % 25143
  \author{V.~I.~Zhukova}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2387
% \author{V.~Zhulanov}\affiliation{\instBINP}\affiliation{\instNSU} % 4983
  \author{R.~\v{Z}leb\v{c}\'{i}k}\affiliation{\instPrague} % 13403
% \author{S.~Zou}\affiliation{\instFudan} % 19363
\collaboration{The Belle II Collaboration}


==> authors-orcid.tex <==
%%% Paper:    B to pi0 pi0
%%% Journal:  Physical Review Letters
%%% Contacts: F. Pham, M. Sevior
%%% ====================================================================
%%% Use \input{pub013-orcid} to insert this material into your latex file.
  \author{F.~Abudin{\'e}n\,\orcidlink{0000-0002-6737-3528}} % 2250
  \author{I.~Adachi\,\orcidlink{0000-0003-2287-0173}} % 2590
  \author{K.~Adamczyk\,\orcidlink{0000-0001-6208-0876}} % 2239
  \author{L.~Aggarwal\,\orcidlink{0000-0002-0909-7537}} % 10083
% \author{P.~Ahlburg\,\orcidlink{0000-0002-9832-7604}} % 2367
  \author{H.~Ahmed\,\orcidlink{0000-0003-3976-7498}} % 11323
% \author{J.~K.~Ahn\,\orcidlink{0000-0002-5795-2243}} % 7423
  \author{H.~Aihara\,\orcidlink{0000-0002-1907-5964}} % 2223
  \author{N.~Akopov\,\orcidlink{0000-0002-4425-2096}} % 9443
  \author{A.~Aloisio\,\orcidlink{0000-0002-3883-6693}} % 2194
% \author{F.~Ameli\,\orcidlink{0000-0001-5435-0450}} % 4683
% \author{L.~Andricek\,\orcidlink{0000-0003-1755-4475}} % 2098
  \author{N.~Anh~Ky\,\orcidlink{0000-0003-0471-197X}} % 2218
  \author{D.~M.~Asner\,\orcidlink{0000-0002-1586-5790}} % 4684
  \author{H.~Atmacan\,\orcidlink{0000-0003-2435-501X}} % 2538
% \author{V.~Aulchenko\,\orcidlink{0000-0002-5394-4406}} % 8183
  \author{T.~Aushev\,\orcidlink{0000-0002-6347-7055}} % 3747
  \author{V.~Aushev\,\orcidlink{0000-0002-8588-5308}} % 2155
% \author{T.~Aziz\,\orcidlink{-}} % 3523
% \author{V.~Babu\,\orcidlink{0000-0003-0419-6912}} % 5623
% \author{S.~Bacher\,\orcidlink{0000-0002-2656-2330}} % 2258
  \author{H.~Bae\,\orcidlink{0000-0003-1393-8631}} % 10863
% \author{S.~Baehr\,\orcidlink{0000-0001-7486-3894}} % 2515
  \author{S.~Bahinipati\,\orcidlink{0000-0002-3744-5332}} % 2332
% \author{A.~M.~Bakich\,\orcidlink{0000-0001-8315-4854}} % 2115
  \author{P.~Bambade\,\orcidlink{0000-0001-7378-4852}} % 3003
  \author{Sw.~Banerjee\,\orcidlink{0000-0001-8852-2409}} % 8603
  \author{S.~Bansal\,\orcidlink{0000-0003-1992-0336}} % 5163
  \author{M.~Barrett\,\orcidlink{0000-0002-2095-603X}} % 2180
% \author{G.~Batignani\,\orcidlink{0000-0003-3917-3104}} % 6643
  \author{J.~Baudot\,\orcidlink{0000-0001-5585-0991}} % 2562
  \author{M.~Bauer\,\orcidlink{0000-0002-0953-7387}} % 9863
  \author{A.~Baur\,\orcidlink{0000-0003-1360-3292}} % 5683
  \author{A.~Beaubien\,\orcidlink{0000-0001-9438-089X}} % 6683
% \author{A.~Beaulieu\,\orcidlink{-}} % 2444
  \author{J.~Becker\,\orcidlink{0000-0002-5082-5487}} % 5403
  \author{P.~K.~Behera\,\orcidlink{0000-0002-1527-2266}} % 4204
  \author{J.~V.~Bennett\,\orcidlink{0000-0002-5440-2668}} % 2454
  \author{E.~Bernieri\,\orcidlink{0000-0002-4787-2047}} % 4483
  \author{F.~U.~Bernlochner\,\orcidlink{0000-0001-8153-2719}} % 2282
  \author{V.~Bertacchi\,\orcidlink{0000-0001-9971-1176}} % 2212
  \author{M.~Bertemes\,\orcidlink{0000-0001-5038-360X}} % 2595
  \author{E.~Bertholet\,\orcidlink{0000-0002-3792-2450}} % 13163
  \author{M.~Bessner\,\orcidlink{0000-0003-1776-0439}} % 3783
  \author{S.~Bettarini\,\orcidlink{0000-0001-7742-2998}} % 2350
  \author{V.~Bhardwaj\,\orcidlink{0000-0001-8857-8621}} % 2228
  \author{B.~Bhuyan\,\orcidlink{0000-0001-6254-3594}} % 2097
  \author{F.~Bianchi\,\orcidlink{0000-0002-1524-6236}} % 2564
  \author{T.~Bilka\,\orcidlink{0000-0003-1449-6986}} % 2484
  \author{S.~Bilokin\,\orcidlink{0000-0003-0017-6260}} % 3623
  \author{D.~Biswas\,\orcidlink{0000-0002-7543-3471}} % 8703
% \author{A.~Bobrov\,\orcidlink{0000-0001-5735-8386}} % 2294
  \author{D.~Bodrov\,\orcidlink{0000-0001-5279-4787}} % 9643
  \author{A.~Bolz\,\orcidlink{0000-0002-4033-9223}} % 15403
% \author{A.~Bondar\,\orcidlink{0000-0002-5089-5338}} % 4643
% \author{G.~Bonvicini\,\orcidlink{0000-0003-4861-7918}} % 2095
  \author{J.~Borah\,\orcidlink{0000-0003-2990-1913}} % 7083
  \author{A.~Bozek\,\orcidlink{0000-0002-5915-1319}} % 2303
  \author{M.~Bra\v{c}ko\,\orcidlink{0000-0002-2495-0524}} % 2425
  \author{P.~Branchini\,\orcidlink{0000-0002-2270-9673}} % 2577
% \author{N.~Braun\,\orcidlink{0000-0002-6969-5635}} % 2436
  \author{R.~A.~Briere\,\orcidlink{0000-0001-5229-1039}} % 2584
  \author{T.~E.~Browder\,\orcidlink{0000-0001-7357-9007}} % 2560
% \author{D.~N.~Brown\,\orcidlink{0000-0002-9635-4174}} % 8743
  \author{A.~Budano\,\orcidlink{0000-0002-0856-1131}} % 2171
% \author{L.~Burmistrov\,\orcidlink{-}} % 2111
  \author{S.~Bussino\,\orcidlink{0000-0002-3829-9592}} % 5384
  \author{M.~Campajola\,\orcidlink{0000-0003-2518-7134}} % 5223
  \author{L.~Cao\,\orcidlink{0000-0001-8332-5668}} % 2099
  \author{G.~Casarosa\,\orcidlink{0000-0003-4137-938X}} % 2491
  \author{C.~Cecchi\,\orcidlink{0000-0002-2192-8233}} % 2433
% \author{J.~Cerasoli\,\orcidlink{0000-0001-9777-881X}} % 20746
% \author{D.~\v{C}ervenkov\,\orcidlink{0000-0002-1865-741X}} % 2078
  \author{M.-C.~Chang\,\orcidlink{0000-0002-8650-6058}} % 2827
  \author{P.~Chang\,\orcidlink{0000-0003-4064-388X}} % 2542
  \author{R.~Cheaib\,\orcidlink{0000-0001-5729-8926}} % 2208
  \author{P.~Cheema\,\orcidlink{0000-0001-8472-5727}} % 15264
  \author{V.~Chekelian\,\orcidlink{0000-0001-8860-8288}} % 2167
  \author{C.~Chen\,\orcidlink{0000-0003-1589-9955}} % 12803
% \author{Y.~Q.~Chen\,\orcidlink{0000-0002-2057-1076}} % 2576
  \author{Y.~Q.~Chen\,\orcidlink{0000-0002-7285-3251}} % 16264
% \author{Y.-T.~Chen\,\orcidlink{0000-0003-2639-2850}} % 2884
  \author{B.~G.~Cheon\,\orcidlink{0000-0002-8803-4429}} % 2173
  \author{K.~Chilikin\,\orcidlink{0000-0001-7620-2053}} % 2308
  \author{K.~Chirapatpimol\,\orcidlink{0000-0003-2099-7760}} % 10803
  \author{H.-E.~Cho\,\orcidlink{0000-0002-7008-3759}} % 2182
  \author{K.~Cho\,\orcidlink{0000-0003-1705-7399}} % 2516
  \author{S.-J.~Cho\,\orcidlink{0000-0002-1673-5664}} % 2723
  \author{S.-K.~Choi\,\orcidlink{0000-0003-2747-8277}} % 2364
  \author{S.~Choudhury\,\orcidlink{0000-0001-9841-0216}} % 2206
  \author{D.~Cinabro\,\orcidlink{0000-0001-7347-6585}} % 2092
  \author{J.~Cochran\,\orcidlink{0000-0002-1492-914X}} % 12604
  \author{L.~Corona\,\orcidlink{0000-0002-2577-9909}} % 3944
% \author{L.~M.~Cremaldi\,\orcidlink{0000-0001-5550-7827}} % 2276
  \author{S.~Cunliffe\,\orcidlink{0000-0003-0167-8641}} % 2272
% \author{T.~Czank\,\orcidlink{0000-0001-6621-3373}} % 2254
  \author{S.~Das\,\orcidlink{0000-0001-6857-966X}} % 9163
% \author{N.~Dash\,\orcidlink{0000-0003-2172-3534}} % 2601
  \author{F.~Dattola\,\orcidlink{0000-0003-3316-8574}} % 3745
  \author{E.~De~La~Cruz-Burelo\,\orcidlink{0000-0002-7469-6974}} % 2359
  \author{S.~A.~De~La~Motte\,\orcidlink{0000-0003-3905-6805}} % 2128
  \author{G.~de~Marino\,\orcidlink{0000-0002-6509-7793}} % 8364
  \author{G.~De~Nardo\,\orcidlink{0000-0002-2047-9675}} % 2459
  \author{M.~De~Nuccio\,\orcidlink{0000-0002-0972-9047}} % 2610
  \author{G.~De~Pietro\,\orcidlink{0000-0001-8442-107X}} % 2528
  \author{R.~de~Sangro\,\orcidlink{0000-0002-3808-5455}} % 2524
% \author{B.~Deschamps\,\orcidlink{0000-0003-2497-5008}} % 2671
  \author{M.~Destefanis\,\orcidlink{0000-0003-1997-6751}} % 2594
  \author{S.~Dey\,\orcidlink{0000-0003-2997-3829}} % 5023
  \author{A.~De~Yta-Hernandez\,\orcidlink{0000-0002-2162-7334}} % 2104
  \author{R.~Dhamija\,\orcidlink{0000-0001-7052-3163}} % 9465
  \author{A.~Di~Canto\,\orcidlink{0000-0003-1233-3876}} % 10963
  \author{F.~Di~Capua\,\orcidlink{0000-0001-9076-5936}} % 2065
% \author{S.~Di~Carlo\,\orcidlink{0000-0002-4570-3135}} % 2079
% \author{J.~Dingfelder\,\orcidlink{0000-0001-5767-2121}} % 2151
  \author{Z.~Dole\v{z}al\,\orcidlink{0000-0002-5662-3675}} % 2319
  \author{I.~Dom\'{\i}nguez~Jim\'{e}nez\,\orcidlink{0000-0001-6831-3159}} % 2191
  \author{T.~V.~Dong\,\orcidlink{0000-0003-3043-1939}} % 2215
  \author{M.~Dorigo\,\orcidlink{0000-0002-0681-6946}} % 12543
  \author{K.~Dort\,\orcidlink{0000-0003-0849-8774}} % 5583
  \author{D.~Dossett\,\orcidlink{0000-0002-5670-5582}} % 2574
  \author{S.~Dreyer\,\orcidlink{0000-0002-6295-100X}} % 12823
  \author{S.~Dubey\,\orcidlink{0000-0002-1345-0970}} % 11063
% \author{S.~Duell\,\orcidlink{0000-0001-9918-9808}} % 2344
  \author{G.~Dujany\,\orcidlink{0000-0002-1345-8163}} % 9703
  \author{P.~Ecker\,\orcidlink{0000-0002-6817-6868}} % 5563
  \author{M.~Eliachevitch\,\orcidlink{0000-0003-2033-537X}} % 2725
% \author{D.~Epifanov\,\orcidlink{0000-0001-8656-2693}} % 2551
  \author{P.~Feichtinger\,\orcidlink{0000-0003-3966-7497}} % 9843
  \author{T.~Ferber\,\orcidlink{0000-0002-6849-0427}} % 2482
  \author{D.~Ferlewicz\,\orcidlink{0000-0002-4374-1234}} % 2073
  \author{T.~Fillinger\,\orcidlink{0000-0001-9795-7412}} % 9803
  \author{C.~Finck\,\orcidlink{0000-0002-5068-5453}} % 15803
  \author{G.~Finocchiaro\,\orcidlink{0000-0002-3936-2151}} % 2400
% \author{P.~Fischer\,\orcidlink{0000-0002-9808-3574}} % 2141
% \author{K.~Flood\,\orcidlink{0000-0002-3463-6571}} % 12103
  \author{A.~Fodor\,\orcidlink{0000-0002-2821-759X}} % 2312
  \author{F.~Forti\,\orcidlink{0000-0001-6535-7965}} % 2432
  \author{A.~Frey\,\orcidlink{0000-0001-7470-3874}} % 2150
% \author{M.~Friedl\,\orcidlink{0000-0002-7420-2559}} % 2442
  \author{B.~G.~Fulsom\,\orcidlink{0000-0002-5862-9739}} % 2563
% \author{M.~Gabriel\,\orcidlink{-}} % 2443
  \author{A.~Gabrielli\,\orcidlink{0000-0001-7695-0537}} % 13523
% \author{N.~Gabyshev\,\orcidlink{0000-0002-8593-6857}} % 2510
  \author{E.~Ganiev\,\orcidlink{0000-0001-8346-8597}} % 4623
  \author{M.~Garcia-Hernandez\,\orcidlink{0000-0003-2393-3367}} % 4823
% \author{R.~Garg\,\orcidlink{0000-0002-7406-4707}} % 2213
% \author{A.~Garmash\,\orcidlink{0000-0003-2599-1405}} % 2161
  \author{G.~Gaudino\,\orcidlink{0000-0001-5983-1552}} % 16563
  \author{V.~Gaur\,\orcidlink{0000-0002-8880-6134}} % 2413
% \author{A.~Gaz\,\orcidlink{0000-0001-6754-3315}} % 2181
% \author{U.~Gebauer\,\orcidlink{0000-0002-5679-2209}} % 2174
  \author{A.~Gellrich\,\orcidlink{0000-0003-0974-6231}} % 2480
% \author{J.~Gemmler\,\orcidlink{-}} % 2321
% \author{T.~Ge{\ss}ler\,\orcidlink{-}} % 2121
  \author{G.~Ghevondyan\,\orcidlink{0000-0003-0096-3555}} % 9445
% \author{G.~Giakoustidis\,\orcidlink{0000-0001-5982-1784}} % 13723
  \author{R.~Giordano\,\orcidlink{0000-0002-5496-7247}} % 2103
  \author{A.~Giri\,\orcidlink{0000-0002-8895-0128}} % 2106
% \author{A.~Glazov\,\orcidlink{0000-0002-8553-7338}} % 2473
  \author{B.~Gobbo\,\orcidlink{0000-0002-3147-4562}} % 2109
  \author{R.~Godang\,\orcidlink{0000-0002-8317-0579}} % 2449
  \author{P.~Goldenzweig\,\orcidlink{0000-0001-8785-847X}} % 2345
% \author{B.~Golob\,\orcidlink{0000-0001-9632-5616}} % 3703
% \author{P.~Gomis\,\orcidlink{0000-0002-9072-9406}} % 2354
% \author{G.~Gong\,\orcidlink{0000-0001-7192-1833}} % 2727
% \author{P.~Grace\,\orcidlink{0000-0001-9005-7403}} % 9563
  \author{W.~Gradl\,\orcidlink{0000-0002-9974-8320}} % 2570
  \author{T.~Grammatico\,\orcidlink{0000-0002-2818-9744}} % 20623
  \author{S.~Granderath\,\orcidlink{0000-0002-9945-463X}} % 8383
  \author{E.~Graziani\,\orcidlink{0000-0001-8602-5652}} % 2342
  \author{D.~Greenwald\,\orcidlink{0000-0001-6964-8399}} % 2686
  \author{Z.~Gruberov\'{a}\,\orcidlink{0000-0002-5691-1044}} % 8824
  \author{T.~Gu\,\orcidlink{0000-0002-1470-6536}} % 14283
  \author{Y.~Guan\,\orcidlink{0000-0002-5541-2278}} % 2514
  \author{K.~Gudkova\,\orcidlink{0000-0002-5858-3187}} % 10504
  \author{J.~Guilliams\,\orcidlink{0000-0001-8229-3975}} % 13543
% \author{C.~Hadjivasiliou\,\orcidlink{0000-0002-2234-0001}} % 9503
  \author{S.~Halder\,\orcidlink{0000-0002-6280-494X}} % 4743
% \author{K.~Hara\,\orcidlink{0000-0002-5361-1871}} % 2462
  \author{T.~Hara\,\orcidlink{0000-0002-4321-0417}} % 2523
% \author{O.~Hartbrich\,\orcidlink{0000-0001-7741-4381}} % 2158
  \author{K.~Hayasaka\,\orcidlink{0000-0002-6347-433X}} % 2330
  \author{H.~Hayashii\,\orcidlink{0000-0002-5138-5903}} % 2455
  \author{S.~Hazra\,\orcidlink{0000-0001-6954-9593}} % 7663
  \author{C.~Hearty\,\orcidlink{0000-0001-6568-0252}} % 2450
  \author{M.~T.~Hedges\,\orcidlink{0000-0001-6504-1872}} % 2265
  \author{I.~Heredia~de~la~Cruz\,\orcidlink{0000-0002-8133-6467}} % 2559
  \author{M.~Hern\'{a}ndez~Villanueva\,\orcidlink{0000-0002-6322-5587}} % 2466
  \author{A.~Hershenhorn\,\orcidlink{0000-0001-8753-5451}} % 2552
  \author{T.~Higuchi\,\orcidlink{0000-0002-7761-3505}} % 2485
  \author{E.~C.~Hill\,\orcidlink{0000-0002-1725-7414}} % 7823
% \author{H.~Hirata\,\orcidlink{0000-0001-9005-4616}} % 2070
% \author{M.~Hoek\,\orcidlink{0000-0002-1893-8764}} % 2101
  \author{M.~Hohmann\,\orcidlink{0000-0001-5147-4781}} % 2077
% \author{S.~Hollitt\,\orcidlink{0000-0002-4962-3546}} % 2557
% \author{T.~Hotta\,\orcidlink{0000-0002-1079-5826}} % 2084
  \author{C.-L.~Hsu\,\orcidlink{0000-0002-1641-430X}} % 2299
% \author{K.~Huang\,\orcidlink{0000-0001-9342-7406}} % 2389
  \author{T.~Humair\,\orcidlink{0000-0002-2922-9779}} % 10643
  \author{T.~Iijima\,\orcidlink{0000-0002-4271-711X}} % 2446
  \author{K.~Inami\,\orcidlink{0000-0003-2765-7072}} % 2323
  \author{G.~Inguglia\,\orcidlink{0000-0003-0331-8279}} % 2500
  \author{N.~Ipsita\,\orcidlink{0000-0002-2927-3366}} % 12223
% \author{J.~Irakkathil~Jabbar\,\orcidlink{0000-0001-7948-1633}} % 7343
  \author{A.~Ishikawa\,\orcidlink{0000-0002-3561-5633}} % 2281
  \author{S.~Ito\,\orcidlink{0000-0003-2737-8145}} % 17463
  \author{R.~Itoh\,\orcidlink{0000-0003-1590-0266}} % 2487
  \author{M.~Iwasaki\,\orcidlink{0000-0002-9402-7559}} % 2360
% \author{Y.~Iwasaki\,\orcidlink{0000-0001-7261-2557}} % 2229
% \author{S.~Iwata\,\orcidlink{-}} % 4323
  \author{P.~Jackson\,\orcidlink{0000-0002-0847-402X}} % 2255
  \author{W.~W.~Jacobs\,\orcidlink{0000-0002-9996-6336}} % 2322
  \author{D.~E.~Jaffe\,\orcidlink{0000-0003-3122-4384}} % 3663
  \author{E.-J.~Jang\,\orcidlink{0000-0002-1935-9887}} % 6744
% \author{M.~Jeandron\,\orcidlink{-}} % 2806
% \author{H.~B.~Jeon\,\orcidlink{0000-0002-0857-0353}} % 2170
  \author{Q.~P.~Ji\,\orcidlink{0000-0003-2963-2565}} % 16243
  \author{S.~Jia\,\orcidlink{0000-0001-8176-8545}} % 2457
  \author{Y.~Jin\,\orcidlink{0000-0002-7323-0830}} % 2105
% \author{C.~Joo\,\orcidlink{-}} % 3525
  \author{K.~K.~Joo\,\orcidlink{0000-0002-5515-0087}} % 4224
  \author{H.~Junkerkalefeld\,\orcidlink{0000-0003-3987-9895}} % 12963
% \author{I.~Kadenko\,\orcidlink{0000-0001-8766-4229}} % 3843
% \author{J.~Kahn\,\orcidlink{0000-0002-8517-2359}} % 2448
  \author{H.~Kakuno\,\orcidlink{0000-0002-9957-6055}} % 2391
  \author{M.~Kaleta\,\orcidlink{0000-0002-2863-5476}} % 5603
% \author{D.~Kalita\,\orcidlink{0000-0003-3054-1222}} % 2220
  \author{A.~B.~Kaliyar\,\orcidlink{0000-0002-2211-619X}} % 7344
  \author{J.~Kandra\,\orcidlink{0000-0001-5635-1000}} % 2541
  \author{K.~H.~Kang\,\orcidlink{0000-0002-6816-0751}} % 2283
  \author{S.~Kang\,\orcidlink{0000-0002-5320-7043}} % 12683
% \author{P.~Kapusta\,\orcidlink{0000-0003-1235-1935}} % 6663
  \author{R.~Karl\,\orcidlink{0000-0002-3619-0876}} % 10923
  \author{G.~Karyan\,\orcidlink{0000-0001-5365-3716}} % 2550
% \author{Y.~Kato\,\orcidlink{0000-0001-6314-4288}} % 2549
% \author{H.~Kawai\,\orcidlink{-}} % 4344
  \author{T.~Kawasaki\,\orcidlink{0000-0002-4089-5238}} % 4363
% \author{C.~Ketter\,\orcidlink{0000-0002-5161-9722}} % 2236
% \author{H.~Kichimi\,\orcidlink{0000-0003-0534-4710}} % 2233
  \author{C.~Kiesling\,\orcidlink{0000-0002-2209-535X}} % 2168
  \author{C.-H.~Kim\,\orcidlink{0000-0002-5743-7698}} % 2358
  \author{D.~Y.~Kim\,\orcidlink{0000-0001-8125-9070}} % 2315
% \author{H.~J.~Kim\,\orcidlink{0000-0001-9787-4684}} % 4863
  \author{K.-H.~Kim\,\orcidlink{0000-0002-4659-1112}} % 2118
% \author{K.~Kim\,\orcidlink{-}} % 2409
% \author{S.-H.~Kim\,\orcidlink{-}} % 2428
  \author{Y.-K.~Kim\,\orcidlink{0000-0002-9695-8103}} % 2379
% \author{Y.~J.~Kim\,\orcidlink{0000-0001-9511-9634}} % 2403
% \author{T.~D.~Kimmel\,\orcidlink{0000-0002-9743-8249}} % 2241
  \author{H.~Kindo\,\orcidlink{0000-0002-6756-3591}} % 2195
  \author{K.~Kinoshita\,\orcidlink{0000-0001-7175-4182}} % 2318
% \author{C.~Kleinwort\,\orcidlink{0000-0002-9017-9504}} % 2499
% \author{B.~Knysh\,\orcidlink{-}} % 8883
  \author{P.~Kody\v{s}\,\orcidlink{0000-0002-8644-2349}} % 2407
  \author{T.~Koga\,\orcidlink{0000-0002-1644-2001}} % 6963
  \author{S.~Kohani\,\orcidlink{0000-0003-3869-6552}} % 9143
  \author{K.~Kojima\,\orcidlink{0000-0002-3638-0266}} % 6363
% \author{I.~Komarov\,\orcidlink{0000-0001-6282-1881}} % 2210
  \author{T.~Konno\,\orcidlink{0000-0003-2487-8080}} % 2490
  \author{A.~Korobov\,\orcidlink{0000-0001-5959-8172}} % 4185
  \author{S.~Korpar\,\orcidlink{0000-0003-0971-0968}} % 2475
% \author{E.~Kou\,\orcidlink{0000-0002-8650-6699}} % 3765
% \author{N.~Kovalchuk\,\orcidlink{0000-0002-5696-5077}} % 6964
  \author{E.~Kovalenko\,\orcidlink{0000-0001-8084-1931}} % 3884
  \author{R.~Kowalewski\,\orcidlink{0000-0002-7314-0990}} % 2293
  \author{T.~M.~G.~Kraetzschmar\,\orcidlink{0000-0001-8395-2928}} % 7543
% \author{F.~Krinner\,\orcidlink{-}} % 9383
  \author{P.~Kri\v{z}an\,\orcidlink{0000-0002-4967-7675}} % 2474
% \author{R.~Kroeger\,\orcidlink{-}} % 2242
% \author{J.~F.~Krohn\,\orcidlink{0000-0002-5001-0675}} % 2502
  \author{P.~Krokovny\,\orcidlink{0000-0002-1236-4667}} % 2575
% \author{H.~Kr\"uger\,\orcidlink{0000-0001-8287-3961}} % 2290
% \author{W.~Kuehn\,\orcidlink{0000-0001-6018-9878}} % 2534
  \author{T.~Kuhr\,\orcidlink{0000-0001-6251-8049}} % 2486
  \author{J.~Kumar\,\orcidlink{0000-0002-8465-433X}} % 6464
% \author{M.~Kumar\,\orcidlink{0000-0002-6627-9708}} % 2744
  \author{R.~Kumar\,\orcidlink{0000-0002-6277-2626}} % 2189
  \author{K.~Kumara\,\orcidlink{0000-0003-1572-5365}} % 2257
% \author{T.~Kumita\,\orcidlink{0000-0001-7572-4538}} % 4083
  \author{T.~Kunigo\,\orcidlink{0000-0001-9613-2849}} % 10104
% \author{M.~K\"{u}nzel\,\orcidlink{-}} % 2139
% \author{S.~Kurz\,\orcidlink{0000-0002-1797-5774}} % 9363
  \author{A.~Kuzmin\,\orcidlink{0000-0002-7011-5044}} % 2520
% \author{P.~Kvasni\v{c}ka\,\orcidlink{0000-0001-6281-0648}} % 2184
  \author{Y.-J.~Kwon\,\orcidlink{0000-0001-9448-5691}} % 2231
  \author{S.~Lacaprara\,\orcidlink{0000-0002-0551-7696}} % 2447
% \author{Y.-T.~Lai\,\orcidlink{0000-0001-9553-3421}} % 2066
% \author{C.~La~Licata\,\orcidlink{0000-0002-8946-8202}} % 2348
% \author{K.~Lalwani\,\orcidlink{0000-0002-7294-396X}} % 2142
  \author{T.~Lam\,\orcidlink{0000-0001-9128-6806}} % 2729
  \author{L.~Lanceri\,\orcidlink{0000-0001-8220-3095}} % 2540
  \author{J.~S.~Lange\,\orcidlink{0000-0003-0234-0474}} % 2277
  \author{M.~Laurenza\,\orcidlink{0000-0002-7400-6013}} % 10223
  \author{K.~Lautenbach\,\orcidlink{0000-0003-3762-694X}} % 2102
% \author{P.~J.~Laycock\,\orcidlink{0000-0002-8572-5339}} % 7683
  \author{R.~Leboucher\,\orcidlink{0000-0003-3097-6613}} % 14083
  \author{F.~R.~Le~Diberder\,\orcidlink{0000-0002-9073-5689}} % 3267
% \author{I.-S.~Lee\,\orcidlink{0000-0002-7786-323X}} % 2422
% \author{S.~C.~Lee\,\orcidlink{0000-0002-9835-1006}} % 2544
  \author{P.~Leitl\,\orcidlink{0000-0002-1336-9558}} % 2414
% \author{D.~Levit\,\orcidlink{0000-0001-5789-6205}} % 2507
% \author{P.~M.~Lewis\,\orcidlink{0000-0002-5991-622X}} % 2582
  \author{C.~Li\,\orcidlink{0000-0002-3240-4523}} % 2325
  \author{L.~K.~Li\,\orcidlink{0000-0002-7366-1307}} % 3263
% \author{S.~X.~Li\,\orcidlink{0000-0003-4669-1495}} % 2377
  \author{Y.~B.~Li\,\orcidlink{0000-0002-9909-2851}} % 2573
  \author{J.~Libby\,\orcidlink{0000-0002-1219-3247}} % 2262
  \author{K.~Lieret\,\orcidlink{0000-0003-2792-7511}} % 2268
% \author{J.~Lin\,\orcidlink{0000-0002-3653-2899}} % 2401
  \author{Z.~Liptak\,\orcidlink{0000-0002-6491-8131}} % 3565
  \author{Q.~Y.~Liu\,\orcidlink{0000-0002-7684-0415}} % 7045
% \author{Z.~A.~Liu\,\orcidlink{0000-0002-2896-1386}} % 3283
  \author{Z.~Q.~Liu\,\orcidlink{0000-0002-0290-3022}} % 11303
  \author{D.~Liventsev\,\orcidlink{0000-0003-3416-0056}} % 2578
  \author{S.~Longo\,\orcidlink{0000-0002-8124-8969}} % 2396
% \author{A.~Loos\,\orcidlink{-}} % 2356
  \author{A.~Lozar\,\orcidlink{0000-0002-0569-6882}} % 12423
% \author{P.~Lu\,\orcidlink{-}} % 2148
  \author{T.~Lueck\,\orcidlink{0000-0003-3915-2506}} % 2406
% \author{F.~Luetticke\,\orcidlink{-}} % 2533
% \author{T.~Luo\,\orcidlink{0000-0001-5139-5784}} % 3268
  \author{C.~Lyu\,\orcidlink{0000-0002-2275-0473}} % 12484
% \author{Y.~Ma\,\orcidlink{0000-0001-8412-8308}} % 16883
  \author{M.~Maggiora\,\orcidlink{0000-0003-4143-9127}} % 5343
  \author{S.~P.~Maharana\,\orcidlink{0000-0002-1746-4683}} % 19083
  \author{R.~Maiti\,\orcidlink{0000-0001-5534-7149}} % 12043
  \author{S.~Maity\,\orcidlink{0000-0003-3076-9243}} % 2985
  \author{R.~Manfredi\,\orcidlink{0000-0002-8552-6276}} % 10303
  \author{E.~Manoni\,\orcidlink{0000-0002-9826-7947}} % 2305
  \author{A.~C.~Manthei\,\orcidlink{0000-0002-6900-5729}} % 15023
  \author{M.~Mantovano\,\orcidlink{0000-0002-5979-5050}} % 19783
% \author{D.~Marcantonio\,\orcidlink{0000-0002-1315-8646}} % 11163
  \author{S.~Marcello\,\orcidlink{0000-0003-4144-863X}} % 4223
  \author{C.~Marinas\,\orcidlink{0000-0003-1903-3251}} % 2133
  \author{L.~Martel\,\orcidlink{0000-0001-8562-0038}} % 13503
  \author{C.~Martellini\,\orcidlink{0000-0002-7189-8343}} % 16983
  \author{A.~Martini\,\orcidlink{0000-0003-1161-4983}} % 2336
  \author{T.~Martinov\,\orcidlink{0000-0001-7846-1913}} % 19463
  \author{L.~Massaccesi\,\orcidlink{0000-0003-1762-4699}} % 16323
% \author{M.~Masuda\,\orcidlink{0000-0002-7109-5583}} % 2238
  \author{T.~Matsuda\,\orcidlink{0000-0003-4673-570X}} % 5543
  \author{K.~Matsuoka\,\orcidlink{0000-0003-1706-9365}} % 2316
  \author{D.~Matvienko\,\orcidlink{0000-0002-2698-5448}} % 2351
  \author{S.~K.~Maurya\,\orcidlink{0000-0002-7764-5777}} % 9763
  \author{J.~A.~McKenna\,\orcidlink{0000-0001-9871-9002}} % 2392
% \author{J.~McNeil\,\orcidlink{0000-0002-2481-1014}} % 2382
% \author{F.~Meggendorfer\,\orcidlink{0000-0002-1466-7207}} % 7103
  \author{F.~Meier\,\orcidlink{0000-0002-6088-0412}} % 3103
  \author{M.~Merola\,\orcidlink{0000-0002-7082-8108}} % 2456
  \author{F.~Metzner\,\orcidlink{0000-0002-0128-264X}} % 2296
  \author{M.~Milesi\,\orcidlink{0000-0002-8805-1886}} % 5443
  \author{C.~Miller\,\orcidlink{0000-0003-2631-1790}} % 2273
  \author{K.~Miyabayashi\,\orcidlink{0000-0003-4352-734X}} % 2327
  \author{H.~Miyake\,\orcidlink{0000-0002-7079-8236}} % 2452
% \author{H.~Miyata\,\orcidlink{0000-0002-1026-2894}} % 2071
  \author{R.~Mizuk\,\orcidlink{0000-0002-2209-6969}} % 2483
% \author{K.~Azmi\,\orcidlink{0000-0001-7933-5097}} % 2506
  \author{G.~B.~Mohanty\,\orcidlink{0000-0001-6850-7666}} % 2278
  \author{N.~Molina-Gonzalez\,\orcidlink{0000-0002-0903-1722}} % 8004
  \author{S.~Moneta\,\orcidlink{0000-0003-2184-7510}} % 13303
% \author{H.~Moon\,\orcidlink{0000-0001-5213-6477}} % 2304
% \author{T.~Moon\,\orcidlink{-}} % 2397
% \author{J.~A.~Mora~Grimaldo\,\orcidlink{-}} % 4403
% \author{T.~Morii\,\orcidlink{-}} % 3543
  \author{H.-G.~Moser\,\orcidlink{0000-0003-3579-9951}} % 2120
  \author{M.~Mrvar\,\orcidlink{0000-0001-6388-3005}} % 2527
% \author{F.~J.~M\"{u}ller\,\orcidlink{0000-0002-2011-2881}} % 2123
% \author{Th.~Muller\,\orcidlink{0000-0003-4337-0098}} % 2165
% \author{G.~Muroyama\,\orcidlink{-}} % 2093
% \author{C.~Murphy\,\orcidlink{0000-0002-6441-075X}} % 12403
  \author{R.~Mussa\,\orcidlink{0000-0002-0294-9071}} % 2372
  \author{I.~Nakamura\,\orcidlink{0000-0002-7640-5456}} % 3463
  \author{K.~R.~Nakamura\,\orcidlink{0000-0001-7012-7355}} % 2417
% \author{E.~Nakano\,\orcidlink{0000-0003-2282-5217}} % 2554
  \author{M.~Nakao\,\orcidlink{0000-0001-8424-7075}} % 2498
  \author{H.~Nakayama\,\orcidlink{0000-0002-2030-9967}} % 2232
% \author{H.~Nakazawa\,\orcidlink{0000-0003-1684-6628}} % 2335
  \author{Y.~Nakazawa\,\orcidlink{0000-0002-6271-5808}} % 17383
  \author{A.~Narimani~Charan\,\orcidlink{0000-0002-5975-550X}} % 10143
  \author{M.~Naruki\,\orcidlink{0000-0003-1773-2999}} % 4583
  \author{D.~Narwal\,\orcidlink{0000-0001-6585-7767}} % 7223
  \author{Z.~Natkaniec\,\orcidlink{0000-0003-0486-9291}} % 3923
  \author{A.~Natochii\,\orcidlink{0000-0002-1076-814X}} % 12063
  \author{L.~Nayak\,\orcidlink{0000-0002-7739-914X}} % 9464
  \author{M.~Nayak\,\orcidlink{0000-0002-2572-4692}} % 2371
  \author{G.~Nazaryan\,\orcidlink{0000-0002-9434-6197}} % 9523
% \author{D.~Neverov\,\orcidlink{-}} % 2075
  \author{C.~Niebuhr\,\orcidlink{0000-0002-4375-9741}} % 2477
% \author{M.~Niiyama\,\orcidlink{0000-0003-1746-586X}} % 2063
% \author{J.~Ninkovic\,\orcidlink{0000-0003-1523-3635}} % 2386
  \author{N.~K.~Nisar\,\orcidlink{0000-0001-9562-1253}} % 2522
  \author{S.~Nishida\,\orcidlink{0000-0001-6373-2346}} % 2571
% \author{K.~Nishimura\,\orcidlink{0000-0001-8818-8922}} % 3063
% \author{M.~H.~A.~Nouxman\,\orcidlink{0000-0003-1243-161X}} % 2470
% \author{K.~Ogawa\,\orcidlink{0000-0003-2220-7224}} % 2430
  \author{S.~Ogawa\,\orcidlink{0000-0002-7310-5079}} % 6263
% \author{S.~L.~Olsen\,\orcidlink{0000-0002-6388-9885}} % 4563
% \author{Y.~Onishchuk\,\orcidlink{0000-0002-8261-7543}} % 2157
  \author{H.~Ono\,\orcidlink{0000-0003-4486-0064}} % 2160
  \author{Y.~Onuki\,\orcidlink{0000-0002-1646-6847}} % 2331
  \author{P.~Oskin\,\orcidlink{0000-0002-7524-0936}} % 9623
% \author{F.~Otani\,\orcidlink{0000-0001-6016-219X}} % 16244
% \author{E.~R.~Oxford\,\orcidlink{0000-0002-0813-4578}} % 6943
% \author{H.~Ozaki\,\orcidlink{0000-0001-6901-1881}} % 2984
  \author{P.~Pakhlov\,\orcidlink{0000-0001-7426-4824}} % 2221
  \author{G.~Pakhlova\,\orcidlink{0000-0001-7518-3022}} % 2188
  \author{A.~Paladino\,\orcidlink{0000-0002-3370-259X}} % 2435
% \author{T.~Pang\,\orcidlink{0000-0003-1204-0846}} % 2114
  \author{A.~Panta\,\orcidlink{0000-0001-6385-7712}} % 7943
  \author{E.~Paoloni\,\orcidlink{0000-0001-5969-8712}} % 2488
  \author{S.~Pardi\,\orcidlink{0000-0001-7994-0537}} % 2532
  \author{K.~Parham\,\orcidlink{0000-0001-9556-2433}} % 10684
  \author{H.~Park\,\orcidlink{0000-0001-6087-2052}} % 2284
  \author{J.~Park\,\orcidlink{0000-0001-6520-0028}} % 18203
  \author{S.-H.~Park\,\orcidlink{0000-0001-6019-6218}} % 2509
  \author{B.~Paschen\,\orcidlink{0000-0003-1546-4548}} % 2159
  \author{A.~Passeri\,\orcidlink{0000-0003-4864-3411}} % 2116
% \author{A.~Pathak\,\orcidlink{0000-0001-9861-2942}} % 8723
  \author{S.~Patra\,\orcidlink{0000-0002-4114-1091}} % 3123
  \author{S.~Paul\,\orcidlink{0000-0002-8813-0437}} % 2131
  \author{T.~K.~Pedlar\,\orcidlink{0000-0001-9839-7373}} % 2421
  \author{I.~Peruzzi\,\orcidlink{0000-0001-6729-8436}} % 2253
  \author{R.~Peschke\,\orcidlink{0000-0002-2529-8515}} % 7123
  \author{R.~Pestotnik\,\orcidlink{0000-0003-1804-9470}} % 2476
  \author{F.~Pham\,\orcidlink{0000-0003-0608-2302}} % 2963
  \author{M.~Piccolo\,\orcidlink{0000-0001-9750-0551}} % 2147
  \author{L.~E.~Piilonen\,\orcidlink{0000-0001-6836-0748}} % 2346
  \author{G.~Pinna~Angioni\,\orcidlink{0000-0003-0808-8281}} % 13363
  \author{P.~L.~M.~Podesta-Lerma\,\orcidlink{0000-0002-8152-9605}} % 2266
  \author{T.~Podobnik\,\orcidlink{0000-0002-6131-819X}} % 11223
  \author{S.~Pokharel\,\orcidlink{0000-0002-3367-738X}} % 12283
  \author{L.~Polat\,\orcidlink{0000-0002-2260-8012}} % 9783
% \author{V.~Popov\,\orcidlink{0000-0003-0208-2583}} % 2096
  \author{C.~Praz\,\orcidlink{0000-0002-6154-885X}} % 2726
  \author{S.~Prell\,\orcidlink{0000-0002-0195-8005}} % 12743
  \author{E.~Prencipe\,\orcidlink{0000-0002-9465-2493}} % 2219
  \author{M.~T.~Prim\,\orcidlink{0000-0002-1407-7450}} % 2501
% \author{M.~V.~Purohit\,\orcidlink{0000-0002-8381-8689}} % 2196
  \author{H.~Purwar\,\orcidlink{0000-0002-3876-7069}} % 12363
  \author{N.~Rad\,\orcidlink{0000-0002-5204-0851}} % 11683
  \author{P.~Rados\,\orcidlink{0000-0003-0690-8100}} % 7383
  \author{G.~Raeuber\,\orcidlink{0000-0003-2948-5155}} % 18143
  \author{S.~Raiz\,\orcidlink{0000-0001-7010-8066}} % 13003
  \author{A.~Ramirez~Morales\,\orcidlink{0000-0001-8821-5708}} % 13724
% \author{R.~Rasheed\,\orcidlink{0000-0001-7070-1206}} % 3643
% \author{N.~Rauls\,\orcidlink{0000-0002-6583-4888}} % 11603
  \author{M.~Reif\,\orcidlink{0000-0002-0706-0247}} % 8043
  \author{S.~Reiter\,\orcidlink{0000-0002-6542-9954}} % 2248
  \author{M.~Remnev\,\orcidlink{0000-0001-6975-1724}} % 2785
  \author{I.~Ripp-Baudot\,\orcidlink{0000-0002-1897-8272}} % 2469
% \author{M.~Ritter\,\orcidlink{0000-0001-6507-4631}} % 2580
% \author{M.~Ritzert\,\orcidlink{0000-0003-2928-7044}} % 2526
  \author{G.~Rizzo\,\orcidlink{0000-0003-1788-2866}} % 2579
  \author{L.~B.~Rizzuto\,\orcidlink{0000-0001-6621-6646}} % 3746
  \author{S.~H.~Robertson\,\orcidlink{0000-0003-4096-8393}} % 2471
% \author{P.~Rocchetti\,\orcidlink{0000-0002-2839-3489}} % 13763
  \author{D.~Rodr\'{i}guez~P\'{e}rez\,\orcidlink{0000-0001-8505-649X}} % 2176
% \author{M.~Roehrken\,\orcidlink{0000-0003-0654-2866}} % 11883
  \author{J.~M.~Roney\,\orcidlink{0000-0001-7802-4617}} % 2244
% \author{C.~Rosenfeld\,\orcidlink{0000-0003-3857-1223}} % 2082
  \author{A.~Rostomyan\,\orcidlink{0000-0003-1839-8152}} % 2481
  \author{N.~Rout\,\orcidlink{0000-0002-4310-3638}} % 2965
% \author{M.~Rozanska\,\orcidlink{0000-0003-2651-5021}} % 2205
  \author{G.~Russo\,\orcidlink{0000-0001-5823-4393}} % 2388
% \author{D.~Sahoo\,\orcidlink{0000-0002-5600-9413}} % 2110
% \author{Y.~Sakai\,\orcidlink{0000-0001-9163-3409}} % 2175
  \author{D.~A.~Sanders\,\orcidlink{0000-0002-4902-966X}} % 2458
  \author{S.~Sandilya\,\orcidlink{0000-0002-4199-4369}} % 2286
  \author{A.~Sangal\,\orcidlink{0000-0001-5853-349X}} % 2384
  \author{L.~Santelj\,\orcidlink{0000-0003-3904-2956}} % 2185
% \author{P.~Sartori\,\orcidlink{0000-0002-9528-4338}} % 4523
  \author{Y.~Sato\,\orcidlink{0000-0003-3751-2803}} % 5243
  \author{V.~Savinov\,\orcidlink{0000-0002-9184-2830}} % 2292
  \author{B.~Scavino\,\orcidlink{0000-0003-1771-9161}} % 2518
% \author{J.~Schmitz\,\orcidlink{0000-0001-8274-8124}} % 12863
% \author{M.~Schnepf\,\orcidlink{0000-0003-0623-0184}} % 15683
% \author{M.~Schram\,\orcidlink{-}} % 2306
% \author{H.~Schreeck\,\orcidlink{0000-0002-2287-8047}} % 2434
  \author{J.~Schueler\,\orcidlink{0000-0002-2722-6953}} % 2824
  \author{C.~Schwanda\,\orcidlink{0000-0003-4844-5028}} % 2108
  \author{A.~J.~Schwartz\,\orcidlink{0000-0002-7310-1983}} % 2162
% \author{B.~Schwenker\,\orcidlink{0000-0002-7120-3732}} % 2405
% \author{M.~Schwickardi\,\orcidlink{0000-0003-2033-6700}} % 14743
  \author{Y.~Seino\,\orcidlink{0000-0002-8378-4255}} % 2517
  \author{A.~Selce\,\orcidlink{0000-0001-8228-9781}} % 9043
  \author{K.~Senyo\,\orcidlink{0000-0002-1615-9118}} % 2987
% \author{I.~S.~Seong\,\orcidlink{-}} % 2572
  \author{J.~Serrano\,\orcidlink{0000-0003-2489-7812}} % 12124
  \author{M.~E.~Sevior\,\orcidlink{0000-0002-4824-101X}} % 2328
  \author{C.~Sfienti\,\orcidlink{0000-0002-5921-8819}} % 2214
% \author{W.~Shan\,\orcidlink{0000-0003-2811-2218}} % 11943
  \author{C.~Sharma\,\orcidlink{0000-0002-1312-0429}} % 11584
% \author{V.~Shebalin\,\orcidlink{0000-0003-1012-0957}} % 2339
  \author{C.~P.~Shen\,\orcidlink{0000-0002-9012-4618}} % 2464
  \author{X.~D.~Shi\,\orcidlink{0000-0002-7006-6107}} % 18843
% \author{H.~Shibuya\,\orcidlink{0000-0002-0197-6270}} % 2234
  \author{T.~Shillington\,\orcidlink{0000-0003-3862-4380}} % 7983
% \author{T.~Shimasaki\,\orcidlink{0000-0003-3291-9532}} % 16263
  \author{J.-G.~Shiu\,\orcidlink{0000-0002-8478-5639}} % 2412
% \author{D.~Shtol\,\orcidlink{0000-0002-0622-6065}} % 9223
  \author{B.~Shwartz\,\orcidlink{0000-0002-1456-1496}} % 2122
  \author{A.~Sibidanov\,\orcidlink{0000-0001-8805-4895}} % 2419
  \author{F.~Simon\,\orcidlink{0000-0002-5978-0289}} % 2164
  \author{J.~B.~Singh\,\orcidlink{0000-0001-9029-2462}} % 2903
% \author{S.~Skambraks\,\orcidlink{0000-0001-5919-133X}} % 2394
  \author{J.~Skorupa\,\orcidlink{0000-0002-8566-621X}} % 12523
% \author{K.~Smith\,\orcidlink{0000-0003-0446-9474}} % 2243
  \author{R.~J.~Sobie\,\orcidlink{0000-0001-7430-7599}} % 2472
  \author{A.~Soffer\,\orcidlink{0000-0002-0749-2146}} % 2217
  \author{A.~Sokolov\,\orcidlink{0000-0002-9420-0091}} % 2521
% \author{Y.~Soloviev\,\orcidlink{0000-0003-1136-2827}} % 2479
  \author{E.~Solovieva\,\orcidlink{0000-0002-5735-4059}} % 2398
  \author{S.~Spataro\,\orcidlink{0000-0001-9601-405X}} % 2117
  \author{B.~Spruck\,\orcidlink{0000-0002-3060-2729}} % 2493
  \author{M.~Stari\v{c}\,\orcidlink{0000-0001-8751-5944}} % 2326
  \author{S.~Stefkova\,\orcidlink{0000-0003-2628-530X}} % 8783
  \author{Z.~S.~Stottler\,\orcidlink{0000-0002-1898-5333}} % 2267
  \author{R.~Stroili\,\orcidlink{0000-0002-3453-142X}} % 2465
  \author{J.~Strube\,\orcidlink{0000-0001-7470-9301}} % 2451
% \author{J.~Stypula\,\orcidlink{0000-0002-5844-7476}} % 2368
  \author{Y.~Sue\,\orcidlink{0000-0003-2430-8707}} % 2085
% \author{R.~Sugiura\,\orcidlink{0000-0002-6044-5445}} % 4644
  \author{M.~Sumihama\,\orcidlink{0000-0002-8954-0585}} % 4243
  \author{K.~Sumisawa\,\orcidlink{0000-0001-7003-7210}} % 2583
% \author{T.~Sumiyoshi\,\orcidlink{0000-0002-0486-3896}} % 4184
  \author{W.~Sutcliffe\,\orcidlink{0000-0002-9795-3582}} % 3784
  \author{S.~Y.~Suzuki\,\orcidlink{0000-0002-7135-4901}} % 2496
  \author{H.~Svidras\,\orcidlink{0000-0003-4198-2517}} % 11783
% \author{M.~Tabata\,\orcidlink{0000-0001-6138-1028}} % 2986
% \author{M.~Takahashi\,\orcidlink{0000-0003-1171-5960}} % 2467
  \author{M.~Takizawa\,\orcidlink{0000-0001-8225-3973}} % 2437
  \author{U.~Tamponi\,\orcidlink{0000-0001-6651-0706}} % 2366
% \author{S.~Tanaka\,\orcidlink{0000-0002-6029-6216}} % 2530
  \author{K.~Tanida\,\orcidlink{0000-0002-8255-3746}} % 3803
  \author{H.~Tanigawa\,\orcidlink{0000-0003-3681-9985}} % 2237
% \author{N.~Taniguchi\,\orcidlink{0000-0002-1462-0564}} % 2285
% \author{Y.~Tao\,\orcidlink{-}} % 2362
% \author{P.~Taras\,\orcidlink{-}} % 2202
  \author{F.~Tenchini\,\orcidlink{0000-0003-3469-9377}} % 2546
  \author{A.~Thaller\,\orcidlink{0000-0003-4171-6219}} % 16044
  \author{R.~Tiwary\,\orcidlink{0000-0002-5887-1883}} % 10403
  \author{D.~Tonelli\,\orcidlink{0000-0002-1494-7882}} % 4564
  \author{E.~Torassa\,\orcidlink{0000-0003-2321-0599}} % 2556
  \author{N.~Toutounji\,\orcidlink{0000-0002-1937-6732}} % 2263
  \author{K.~Trabelsi\,\orcidlink{0000-0001-6567-3036}} % 2369
  \author{I.~Tsaklidis\,\orcidlink{0000-0003-3584-4484}} % 13443
% \author{T.~Tsuboyama\,\orcidlink{0000-0002-4575-1997}} % 2361
% \author{N.~Tsuzuki\,\orcidlink{0000-0003-1141-1908}} % 2352
  \author{M.~Uchida\,\orcidlink{0000-0003-4904-6168}} % 2370
  \author{I.~Ueda\,\orcidlink{0000-0002-6833-4344}} % 2519
% \author{S.~Uehara\,\orcidlink{0000-0001-7377-5016}} % 2586
  \author{Y.~Uematsu\,\orcidlink{0000-0002-0296-4028}} % 5883
% \author{T.~Ueno\,\orcidlink{0000-0002-9130-2850}} % 4364
  \author{T.~Uglov\,\orcidlink{0000-0002-4944-1830}} % 2252
  \author{K.~Unger\,\orcidlink{0000-0001-7378-6671}} % 9463
  \author{Y.~Unno\,\orcidlink{0000-0003-3355-765X}} % 2420
  \author{K.~Uno\,\orcidlink{0000-0002-2209-8198}} % 14963
  \author{S.~Uno\,\orcidlink{0000-0002-3401-0480}} % 2149
  \author{P.~Urquijo\,\orcidlink{0000-0002-0887-7953}} % 2302
  \author{Y.~Ushiroda\,\orcidlink{0000-0003-3174-403X}} % 2317
% \author{Y.~V.~Usov\,\orcidlink{0000-0003-3144-2920}} % 5003
  \author{S.~E.~Vahsen\,\orcidlink{0000-0003-1685-9824}} % 2251
  \author{R.~van~Tonder\,\orcidlink{0000-0002-7448-4816}} % 2706
  \author{G.~S.~Varner\,\orcidlink{0000-0002-0302-8151}} % 2119
  \author{K.~E.~Varvell\,\orcidlink{0000-0003-1017-1295}} % 2545
  \author{A.~Vinokurova\,\orcidlink{0000-0003-4220-8056}} % 2289
  \author{V.~S.~Vismaya\,\orcidlink{0000-0002-1606-5349}} % 16063
  \author{L.~Vitale\,\orcidlink{0000-0003-3354-2300}} % 2415
  \author{V.~Vobbilisetti\,\orcidlink{0000-0002-4399-5082}} % 7364
% \author{V.~Vorobyev\,\orcidlink{0000-0002-6660-868X}} % 2298
  \author{A.~Vossen\,\orcidlink{0000-0003-0983-4936}} % 2249
% \author{B.~Wach\,\orcidlink{0000-0003-3533-7669}} % 8203
% \author{E.~Waheed\,\orcidlink{0000-0001-7774-0363}} % 2226
  \author{H.~M.~Wakeling\,\orcidlink{0000-0003-4606-7895}} % 3664
  \author{S.~Wallner\,\orcidlink{0000-0002-9105-1625}} % 20363
% \author{K.~Wan\,\orcidlink{-}} % 2591
% \author{W.~Wan~Abdullah\,\orcidlink{0000-0001-5798-9145}} % 2280
% \author{B.~Wang\,\orcidlink{0000-0001-6136-6952}} % 2569
% \author{C.~H.~Wang\,\orcidlink{0000-0001-6760-9839}} % 2224
  \author{E.~Wang\,\orcidlink{0000-0001-6391-5118}} % 10983
  \author{M.-Z.~Wang\,\orcidlink{0000-0002-0979-8341}} % 2074
  \author{X.~L.~Wang\,\orcidlink{0000-0001-5805-1255}} % 2076
  \author{A.~Warburton\,\orcidlink{0000-0002-2298-7315}} % 2347
  \author{M.~Watanabe\,\orcidlink{0000-0001-6917-6694}} % 2309
  \author{S.~Watanuki\,\orcidlink{0000-0002-5241-6628}} % 6843
% \author{J.~Webb\,\orcidlink{0000-0002-5294-6856}} % 2423
% \author{S.~Wehle\,\orcidlink{0000-0002-6168-1829}} % 2489
  \author{M.~Welsch\,\orcidlink{0000-0002-3026-1872}} % 7023
% \author{O.~Werbycka\,\orcidlink{0000-0002-0614-8773}} % 6123
  \author{C.~Wessel\,\orcidlink{0000-0003-0959-4784}} % 2100
  \author{J.~Wiechczynski\,\orcidlink{0000-0002-3151-6072}} % 2604
% \author{P.~Wieduwilt\,\orcidlink{0000-0002-1706-5359}} % 2343
% \author{H.~Windel\,\orcidlink{0000-0001-9472-0786}} % 2081
  \author{E.~Won\,\orcidlink{0000-0002-4245-7442}} % 2410
% \author{L.~J.~Wu\,\orcidlink{0000-0002-3171-2436}} % 2704
% \author{Y.~Xie\,\orcidlink{0000-0002-0170-2798}} % 20383
  \author{X.~P.~Xu\,\orcidlink{0000-0001-5096-1182}} % 4923
  \author{B.~D.~Yabsley\,\orcidlink{0000-0002-2680-0474}} % 3645
  \author{S.~Yamada\,\orcidlink{0000-0002-8858-9336}} % 2492
  \author{W.~Yan\,\orcidlink{0000-0003-0713-0871}} % 2094
  \author{S.~B.~Yang\,\orcidlink{0000-0002-9543-7971}} % 2374
  \author{H.~Ye\,\orcidlink{0000-0003-0552-5490}} % 2537
  \author{J.~Yelton\,\orcidlink{0000-0001-8840-3346}} % 2067
  \author{J.~H.~Yin\,\orcidlink{0000-0002-1479-9349}} % 2365
% \author{M.~Yonenaga\,\orcidlink{-}} % 2411
  \author{Y.~M.~Yook\,\orcidlink{0000-0002-4912-048X}} % 2453
  \author{K.~Yoshihara\,\orcidlink{0000-0002-3656-2326}} % 12663
% \author{T.~Yoshinobu\,\orcidlink{-}} % 2429
  \author{C.~Z.~Yuan\,\orcidlink{0000-0002-1652-6686}} % 2088
  \author{Y.~Yusa\,\orcidlink{0000-0002-4001-9748}} % 2357
  \author{L.~Zani\,\orcidlink{0000-0003-4957-805X}} % 2529
  \author{Y.~Zhai\,\orcidlink{0000-0001-7207-5122}} % 12703
% \author{J.~Z.~Zhang\,\orcidlink{0000-0001-6535-0659}} % 2349
% \author{Y.~Zhang\,\orcidlink{0000-0003-3780-6676}} % 2607
  \author{Y.~Zhang\,\orcidlink{0000-0003-2961-2820}} % 3303
% \author{Z.~Zhang\,\orcidlink{0000-0001-6140-2044}} % 5363
  \author{V.~Zhilich\,\orcidlink{0000-0002-0907-5565}} % 4703
% \author{J.~S.~Zhou\,\orcidlink{0000-0002-6413-4687}} % 12463
  \author{Q.~D.~Zhou\,\orcidlink{0000-0001-5968-6359}} % 7323
  \author{X.~Y.~Zhou\,\orcidlink{0000-0002-0299-4657}} % 2380
  \author{V.~I.~Zhukova\,\orcidlink{0000-0002-8253-641X}} % 2387
% \author{V.~Zhulanov\,\orcidlink{0000-0002-0306-9199}} % 4983
  \author{R.~\v{Z}leb\v{c}\'{i}k\,\orcidlink{0000-0003-1644-8523}} % 13403
\collaboration{The Belle II Collaboration}



==> authors_plain.tex <==
%%% Paper:    B to pi0 pi0
%%% Journal:  Physical Review Letters
%%% Contacts: F. Pham, M. Sevior
%%% ====================================================================
%%% Use \input{pub013} to insert this material into your latex file.
%%%\newcommand{\instSinica}{Academia Sinica, Taipei 11529, Taiwan}
\newcommand{\instCPPM}{Aix Marseille Universit\'{e}, CNRS/IN2P3, CPPM, 13288 Marseille, France}
\newcommand{\instYerevan}{Alikhanyan National Science Laboratory, Yerevan 0036, Armenia}
\newcommand{\instGoettingen}{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen, Germany}
\newcommand{\instBeihang}{Beihang University, Beijing 100191, China}
%%%\newcommand{\instBUAP}{Benemerita Universidad Autonoma de Puebla, Puebla 72570, Mexico}
\newcommand{\instBNL}{Brookhaven National Laboratory, Upton, New York 11973, U.S.A.}
\newcommand{\instBINP}{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090, Russian Federation}
\newcommand{\instCMU}{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, U.S.A.}
\newcommand{\instCinvestavIPN}{Centro de Investigacion y de Estudios Avanzados del Instituto Politecnico Nacional, Mexico City 07360, Mexico}
\newcommand{\instPrague}{Faculty of Mathematics and Physics, Charles University, 121 16 Prague, Czech Republic}
\newcommand{\instChiangMai}{Chiang Mai University, Chiang Mai 50202, Thailand}
\newcommand{\instChiba}{Chiba University, Chiba 263-8522, Japan}
\newcommand{\instChonnam}{Chonnam National University, Gwangju 61186, South Korea}
%%%\newcommand{\instChula}{Chulalongkorn University, Bangkok 10330, Thailand}
\newcommand{\instCAU}{Chung-Ang University, Seoul 06974, South Korea}
\newcommand{\instConacyt}{Consejo Nacional de Ciencia y Tecnolog\'{\i}a, Mexico City 03940, Mexico}
\newcommand{\instDESY}{Deutsches Elektronen--Synchrotron, 22607 Hamburg, Germany}
\newcommand{\instDuke}{Duke University, Durham, North Carolina 27708, U.S.A.}
\newcommand{\instITAR}{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000, Vietnam}
\newcommand{\instRomaENEA}{ENEA Casaccia, I-00123 Roma, Italy}
%%%\newcommand{\instJuelich}{Forschungszentrum J\"{u}lich, 52425 J\"{u}lich, Germany}
\newcommand{\instFuJen}{Department of Physics, Fu Jen Catholic University, Taipei 24205, Taiwan}
\newcommand{\instFudan}{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, China}
\newcommand{\instGifu}{Gifu University, Gifu 501-1193, Japan}
\newcommand{\instSOKENDAI}{The Graduate University for Advanced Studies (Sokendai), Tsukuba 305-0801, Japan}
\newcommand{\instMainz}{Institut f\"{u}r Kernphysik, Johannes Gutenberg-Universit\"{a}t Mainz, D-55099 Mainz, Germany}
\newcommand{\instGyeongsang}{Gyeongsang National University, Jinju 52828, South Korea}
\newcommand{\instHanyang}{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763, South Korea}
\newcommand{\instHeidelberg}{Heidelberg University, 68131 Mannheim, Germany}
\newcommand{\instHNU}{Henan Normal University, Xinxiang 453007, China}
\newcommand{\instKEK}{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\newcommand{\instJPARC}{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\newcommand{\instHiroshima}{Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8530, Japan}
\newcommand{\instHUNNU}{Hunan Normal University, Changsha 410081, China}
\newcommand{\instFrascati}{INFN Laboratori Nazionali di Frascati, I-00044 Frascati, Italy}
\newcommand{\instNapoliINFN}{INFN Sezione di Napoli, I-80126 Napoli, Italy}
\newcommand{\instPadovaINFN}{INFN Sezione di Padova, I-35131 Padova, Italy}
\newcommand{\instPerugiaINFN}{INFN Sezione di Perugia, I-06123 Perugia, Italy}
\newcommand{\instPisaINFN}{INFN Sezione di Pisa, I-56127 Pisa, Italy}
\newcommand{\instRomaINFN}{INFN Sezione di Roma, I-00185 Roma, Italy}
\newcommand{\instRomaTreINFN}{INFN Sezione di Roma Tre, I-00146 Roma, Italy}
\newcommand{\instTorinoINFN}{INFN Sezione di Torino, I-10125 Torino, Italy}
\newcommand{\instTriesteINFN}{INFN Sezione di Trieste, I-34127 Trieste, Italy}
\newcommand{\instIISER}{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306, India}
\newcommand{\instIITBhubaneswar}{Indian Institute of Technology Bhubaneswar, Bhubaneswar 752050, India}
\newcommand{\instIITGuwahati}{Indian Institute of Technology Guwahati, Assam 781039, India}
\newcommand{\instIITHyderabad}{Indian Institute of Technology Hyderabad, Telangana 502285, India}
\newcommand{\instIITMadras}{Indian Institute of Technology Madras, Chennai 600036, India}
\newcommand{\instIndiana}{Indiana University, Bloomington, Indiana 47408, U.S.A.}
\newcommand{\instIHEPRussia}{Institute for High Energy Physics, Protvino 142281, Russian Federation}
\newcommand{\instHEPHYVienna}{Institute of High Energy Physics, Vienna 1050, Austria}
\newcommand{\instIHEPChina}{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
%%%\newcommand{\instChennai}{Institute of Mathematical Sciences, Chennai 600113, India}
\newcommand{\instIPP}{Institute of Particle Physics (Canada), Victoria, British Columbia V8W 2Y2, Canada}
\newcommand{\instIOP}{Institute of Physics, Vietnam Academy of Science and Technology (VAST), Hanoi, Vietnam}
\newcommand{\instIFIC}{Instituto de Fisica Corpuscular, Paterna 46980, Spain}
\newcommand{\instISU}{Iowa State University, Ames, Iowa 50011, U.S.A.}
\newcommand{\instJAEA}{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195, Japan}
\newcommand{\instKarlsruhe}{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe, Germany}
%%%\newcommand{\instKennesaw}{Kennesaw State University, Kennesaw, Georgia 30144, U.S.A.}
\newcommand{\instKitasato}{Kitasato University, Sagamihara 252-0373, Japan}
\newcommand{\instKISTI}{Korea Institute of Science and Technology Information, Daejeon 34141, South Korea}
\newcommand{\instKoreaUnivKU}{Korea University, Seoul 02841, South Korea}
\newcommand{\instKSU}{Kyoto Sangyo University, Kyoto 603-8555, Japan}
\newcommand{\instKyotoU}{Kyoto University, Kyoto 606-8501, Japan}
\newcommand{\instKyungpook}{Kyungpook National University, Daegu 41566, South Korea}
\newcommand{\instLNNU}{Liaoning Normal University, Dalian 116029, China}
\newcommand{\instGiessen}{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en, Germany}
\newcommand{\instLuther}{Luther College, Decorah, Iowa 52101, U.S.A.}
\newcommand{\instMNITJaipur}{Malaviya National Institute of Technology Jaipur, Jaipur 302017, India}
\newcommand{\instLMU}{Ludwig Maximilians University, 80539 Munich, Germany}
\newcommand{\instMcGill}{McGill University, Montr\'{e}al, Qu\'{e}bec, H3A 2T8, Canada}
%%%\newcommand{\instMETU}{Middle East Technical University, 06531 Ankara, Turkey}
\newcommand{\instMEPhI}{Moscow Physical Engineering Institute, Moscow 115409, Russian Federation}
\newcommand{\instNagoya}{Graduate School of Science, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNagoyaIAR}{Institute for Advanced Research, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNagoyaKMI}{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602, Japan}
%%%\newcommand{\instNNU}{Nanjing Normal University, Nanjing 210023, China}
\newcommand{\instNaraWu}{Nara Women's University, Nara 630-8506, Japan}
%%%\newcommand{\instUNAM}{National Autonomous University of Mexico, Mexico City, Mexico}
\newcommand{\instHSE}{National Research University Higher School of Economics, Moscow 101000, Russian Federation}
\newcommand{\instNTUTaiwan}{Department of Physics, National Taiwan University, Taipei 10617, Taiwan}
\newcommand{\instNUUTaiwan}{National United University, Miao Li 36003, Taiwan}
\newcommand{\instKrakow}{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342, Poland}
\newcommand{\instNiigata}{Niigata University, Niigata 950-2181, Japan}
\newcommand{\instNSU}{Novosibirsk State University, Novosibirsk 630090, Russian Federation}
\newcommand{\instOkinawa}{Okinawa Institute of Science and Technology, Okinawa 904-0495, Japan}
\newcommand{\instOsakaMetropolitan}{Osaka Metropolitan University, Osaka 558-8585, Japan}
\newcommand{\instRCNP}{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047, Japan}
\newcommand{\instPNNL}{Pacific Northwest National Laboratory, Richland, Washington 99352, U.S.A.}
\newcommand{\instPanjab}{Panjab University, Chandigarh 160014, India}
%%%\newcommand{\instPeking}{Peking University, Beijing 100871, China}
\newcommand{\instMPP}{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen, Germany}
\newcommand{\instMPGHLL}{Semiconductor Laboratory of the Max Planck Society, 81739 M\"{u}nchen, Germany}
\newcommand{\instPanjabPAU}{Punjab Agricultural University, Ludhiana 141004, India}
\newcommand{\instRIKENMSL}{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198, Japan}
%%%\newcommand{\instRIKEN}{Theoretical Research Division, Nishina Center, RIKEN, Saitama 351-0198, Japan}
\newcommand{\instSeoul}{Seoul National University, Seoul 08826, South Korea}
\newcommand{\instShandong}{Shandong University, Jinan 250100, China}
\newcommand{\instKyiv}{Taras Shevchenko National University of Kiev, Kiev, Ukraine}
\newcommand{\instSPU}{Showa Pharmaceutical University, Tokyo 194-8543, Japan}
\newcommand{\instSoochow}{Soochow University, Suzhou 215006, China}
\newcommand{\instSoongsil}{Department of Physics and Origin of Matter and Evolution of Galaxy (OMEG) Institute, Soongsil University, Seoul 06978, South Korea}
\newcommand{\instLjubljanaJSI}{J. Stefan Institute, 1000 Ljubljana, Slovenia}
\newcommand{\instTata}{Tata Institute of Fundamental Research, Mumbai 400005, India}
\newcommand{\instTUM}{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
%%%\newcommand{\instECUTUM}{Excellence Cluster Universe, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
\newcommand{\instTelAviv}{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978, Israel}
\newcommand{\instToho}{Toho University, Funabashi 274-8510, Japan}
\newcommand{\instTohoku}{Department of Physics, Tohoku University, Sendai 980-8578, Japan}
\newcommand{\instTitech}{Tokyo Institute of Technology, Tokyo 152-8550, Japan}
\newcommand{\instTokyoMetropolitan}{Tokyo Metropolitan University, Tokyo 192-0397, Japan}
\newcommand{\instUAS}{Universidad Autonoma de Sinaloa, Sinaloa 80000, Mexico}
%%%\newcommand{\instNapoliUNIVA}{Dipartimento di Agraria, Universit\`{a} di Napoli Federico II, I-80055 Portici (NA), Italy}
\newcommand{\instNapoliUNIV}{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli, Italy}
\newcommand{\instPadovaUNIV}{Dipartimento di Fisica e Astronomia, Universit\`{a} di Padova, I-35131 Padova, Italy}
\newcommand{\instPerugiaUNIV}{Dipartimento di Fisica, Universit\`{a} di Perugia, I-06123 Perugia, Italy}
\newcommand{\instPisaUNIV}{Dipartimento di Fisica, Universit\`{a} di Pisa, I-56127 Pisa, Italy}
%%%\newcommand{\instRomaUNIV}{Universit\`{a} di Roma ``La Sapienza,'' I-00185 Roma, Italy}
\newcommand{\instRomaTreUNIV}{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma, Italy}
\newcommand{\instTorinoUNIV}{Dipartimento di Fisica, Universit\`{a} di Torino, I-10125 Torino, Italy}
\newcommand{\instTriesteUNIV}{Dipartimento di Fisica, Universit\`{a} di Trieste, I-34127 Trieste, Italy}
\newcommand{\instMontreal}{Universit\'{e} de Montr\'{e}al, Physique des Particules, Montr\'{e}al, Qu\'{e}bec, H3C 3J7, Canada}
\newcommand{\instIJCLab}{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\newcommand{\instIPHC}{Universit\'{e} de Strasbourg, CNRS, IPHC, UMR 7178, 67037 Strasbourg, France}
\newcommand{\instAdelaide}{Department of Physics, University of Adelaide, Adelaide, South Australia 5005, Australia}
\newcommand{\instBonn}{University of Bonn, 53115 Bonn, Germany}
\newcommand{\instUBC}{University of British Columbia, Vancouver, British Columbia, V6T 1Z1, Canada}
\newcommand{\instCincinnati}{University of Cincinnati, Cincinnati, Ohio 45221, U.S.A.}
\newcommand{\instFlorida}{University of Florida, Gainesville, Florida 32611, U.S.A.}
%%%\newcommand{\instHamburg}{University of Hamburg, 20148 Hamburg, Germany}
\newcommand{\instHawaii}{University of Hawaii, Honolulu, Hawaii 96822, U.S.A.}
\newcommand{\instLjubljanaUniLJ}{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana, Slovenia}
\newcommand{\instLouisville}{University of Louisville, Louisville, Kentucky 40292, U.S.A.}
\newcommand{\instMalaya}{National Centre for Particle Physics, University of Malaya, 50603 Kuala Lumpur, Malaysia}
\newcommand{\instLjubljanaUM}{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor, Slovenia}
\newcommand{\instMelbourne}{School of Physics, University of Melbourne, Victoria 3010, Australia}
\newcommand{\instMississippi}{University of Mississippi, University, Mississippi 38677, U.S.A.}
\newcommand{\instUOM}{University of Miyazaki, Miyazaki 889-2192, Japan}
\newcommand{\instNovaGorica}{University of Nova Gorica, 5000 Nova Gorica, Slovenia}
\newcommand{\instUPES}{University of Petroleum and Energy Studies, Dehradun 248007, India}
\newcommand{\instPittsburgh}{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, U.S.A.}
\newcommand{\instUSTC}{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026, China}
\newcommand{\instSAlabama}{University of South Alabama, Mobile, Alabama 36688, U.S.A.}
\newcommand{\instSCarolina}{University of South Carolina, Columbia, South Carolina 29208, U.S.A.}
\newcommand{\instSydney}{School of Physics, University of Sydney, New South Wales 2006, Australia}
%%%\newcommand{\instTabuk}{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451, Saudi Arabia}
\newcommand{\instUTokyo}{Department of Physics, University of Tokyo, Tokyo 113-0033, Japan}
\newcommand{\instEri}{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032, Japan}
\newcommand{\instIPMU}{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583, Japan}
\newcommand{\instVictoria}{University of Victoria, Victoria, British Columbia, V8W 3P6, Canada}
\newcommand{\instVPI}{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, U.S.A.}
\newcommand{\instWayneState}{Wayne State University, Detroit, Michigan 48202, U.S.A.}
\newcommand{\instXavier}{St. Francis Xavier University, Antigonish, Nova Scotia, B2G 2W5, Canada}
\newcommand{\instYamagata}{Yamagata University, Yamagata 990-8560, Japan}
\newcommand{\instYonsei}{Yonsei University, Seoul 03722, South Korea}
%%%\newcommand{\instZZU}{Zhengzhou University, Zhengzhou 450001, China}
%%%\affiliation{\instSinica}
\affiliation{\instCPPM}
\affiliation{\instYerevan}
\affiliation{\instGoettingen}
%%%\affiliation{\instBeihang}
%%%\affiliation{\instBUAP}
\affiliation{\instBNL}
\affiliation{\instBINP}
\affiliation{\instCMU}
\affiliation{\instCinvestavIPN}
\affiliation{\instPrague}
\affiliation{\instChiangMai}
%%%\affiliation{\instChiba}
\affiliation{\instChonnam}
%%%\affiliation{\instChula}
\affiliation{\instCAU}
\affiliation{\instConacyt}
\affiliation{\instDESY}
\affiliation{\instDuke}
\affiliation{\instITAR}
\affiliation{\instRomaENEA}
%%%\affiliation{\instJuelich}
\affiliation{\instFuJen}
\affiliation{\instFudan}
\affiliation{\instGifu}
\affiliation{\instSOKENDAI}
\affiliation{\instMainz}
\affiliation{\instGyeongsang}
\affiliation{\instHanyang}
%%%\affiliation{\instHeidelberg}
\affiliation{\instHNU}
\affiliation{\instKEK}
\affiliation{\instJPARC}
\affiliation{\instHiroshima}
\affiliation{\instHUNNU}
\affiliation{\instFrascati}
\affiliation{\instNapoliINFN}
\affiliation{\instPadovaINFN}
\affiliation{\instPerugiaINFN}
\affiliation{\instPisaINFN}
%%%\affiliation{\instRomaINFN}
\affiliation{\instRomaTreINFN}
\affiliation{\instTorinoINFN}
\affiliation{\instTriesteINFN}
\affiliation{\instIISER}
\affiliation{\instIITBhubaneswar}
\affiliation{\instIITGuwahati}
\affiliation{\instIITHyderabad}
\affiliation{\instIITMadras}
\affiliation{\instIndiana}
\affiliation{\instIHEPRussia}
\affiliation{\instHEPHYVienna}
\affiliation{\instIHEPChina}
%%%\affiliation{\instChennai}
\affiliation{\instIPP}
\affiliation{\instIOP}
\affiliation{\instIFIC}
\affiliation{\instISU}
\affiliation{\instJAEA}
\affiliation{\instKarlsruhe}
%%%\affiliation{\instKennesaw}
\affiliation{\instKitasato}
\affiliation{\instKISTI}
\affiliation{\instKoreaUnivKU}
%%%\affiliation{\instKSU}
\affiliation{\instKyotoU}
\affiliation{\instKyungpook}
\affiliation{\instLNNU}
\affiliation{\instGiessen}
\affiliation{\instLuther}
\affiliation{\instMNITJaipur}
\affiliation{\instLMU}
\affiliation{\instMcGill}
%%%\affiliation{\instMETU}
%%%\affiliation{\instMEPhI}
\affiliation{\instNagoya}
\affiliation{\instNagoyaIAR}
\affiliation{\instNagoyaKMI}
%%%\affiliation{\instNNU}
\affiliation{\instNaraWu}
%%%\affiliation{\instUNAM}
\affiliation{\instHSE}
\affiliation{\instNTUTaiwan}
%%%\affiliation{\instNUUTaiwan}
\affiliation{\instKrakow}
\affiliation{\instNiigata}
\affiliation{\instNSU}
%%%\affiliation{\instOkinawa}
\affiliation{\instOsakaMetropolitan}
\affiliation{\instRCNP}
\affiliation{\instPNNL}
\affiliation{\instPanjab}
%%%\affiliation{\instPeking}
\affiliation{\instMPP}
%%%\affiliation{\instMPGHLL}
\affiliation{\instPanjabPAU}
\affiliation{\instRIKENMSL}
%%%\affiliation{\instRIKEN}
%%%\affiliation{\instSeoul}
\affiliation{\instShandong}
\affiliation{\instKyiv}
\affiliation{\instSPU}
\affiliation{\instSoochow}
\affiliation{\instSoongsil}
\affiliation{\instLjubljanaJSI}
\affiliation{\instTata}
\affiliation{\instTUM}
%%%\affiliation{\instECUTUM}
\affiliation{\instTelAviv}
\affiliation{\instToho}
%%%\affiliation{\instTohoku}
\affiliation{\instTitech}
\affiliation{\instTokyoMetropolitan}
\affiliation{\instUAS}
%%%\affiliation{\instNapoliUNIVA}
\affiliation{\instNapoliUNIV}
\affiliation{\instPadovaUNIV}
\affiliation{\instPerugiaUNIV}
\affiliation{\instPisaUNIV}
%%%\affiliation{\instRomaUNIV}
\affiliation{\instRomaTreUNIV}
\affiliation{\instTorinoUNIV}
\affiliation{\instTriesteUNIV}
%%%\affiliation{\instMontreal}
\affiliation{\instIJCLab}
\affiliation{\instIPHC}
\affiliation{\instAdelaide}
\affiliation{\instBonn}
\affiliation{\instUBC}
\affiliation{\instCincinnati}
\affiliation{\instFlorida}
%%%\affiliation{\instHamburg}
\affiliation{\instHawaii}
\affiliation{\instLjubljanaUniLJ}
\affiliation{\instLouisville}
%%%\affiliation{\instMalaya}
\affiliation{\instLjubljanaUM}
\affiliation{\instMelbourne}
\affiliation{\instMississippi}
\affiliation{\instUOM}
%%%\affiliation{\instNovaGorica}
\affiliation{\instUPES}
\affiliation{\instPittsburgh}
\affiliation{\instUSTC}
\affiliation{\instSAlabama}
%%%\affiliation{\instSCarolina}
\affiliation{\instSydney}
%%%\affiliation{\instTabuk}
\affiliation{\instUTokyo}
%%%\affiliation{\instEri}
\affiliation{\instIPMU}
\affiliation{\instVictoria}
\affiliation{\instVPI}
\affiliation{\instWayneState}
\affiliation{\instXavier}
\affiliation{\instYamagata}
\affiliation{\instYonsei}
%%%\affiliation{\instZZU}
  \author{F.~Abudin{\'e}n}\affiliation{\instTriesteINFN} % 2250
  \author{I.~Adachi}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2590
  \author{K.~Adamczyk}\affiliation{\instLjubljanaJSI} % 2239
  \author{L.~Aggarwal}\affiliation{\instPanjab} % 10083
% \author{P.~Ahlburg}\affiliation{\instBonn} % 2367
  \author{H.~Ahmed}\affiliation{\instXavier} % 11323
% \author{J.~K.~Ahn}\affiliation{\instKoreaUnivKU} % 7423
  \author{H.~Aihara}\affiliation{\instUTokyo} % 2223
  \author{N.~Akopov}\affiliation{\instYerevan} % 9443
  \author{A.~Aloisio}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % 2194
% \author{F.~Ameli}\affiliation{\instRomaINFN} % 4683
% \author{L.~Andricek}\affiliation{\instMPGHLL} % 2098
  \author{N.~Anh~Ky}\affiliation{\instIOP} % 2218
  \author{D.~M.~Asner}\affiliation{\instBNL} % 4684
  \author{H.~Atmacan}\affiliation{\instCincinnati} % 2538
% \author{V.~Aulchenko}\affiliation{\instBINP}\affiliation{\instNSU} % 8183
  \author{T.~Aushev}\affiliation{\instHSE} % 3747
  \author{V.~Aushev}\affiliation{\instKyiv} % 2155
% \author{T.~Aziz}\affiliation{\instTata} % 3523
% \author{V.~Babu}\affiliation{\instIPHC} % 5623
% \author{S.~Bacher}\affiliation{\instKrakow} % 2258
  \author{H.~Bae}\affiliation{\instUTokyo} % 10863
% \author{S.~Baehr}\affiliation{\instKarlsruhe} % 2515
  \author{S.~Bahinipati}\affiliation{\instIITBhubaneswar} % 2332
% \author{A.~M.~Bakich}\affiliation{\instSydney} % 2115
  \author{P.~Bambade}\affiliation{\instIJCLab} % 3003
  \author{Sw.~Banerjee}\affiliation{\instLouisville} % 8603
  \author{S.~Bansal}\affiliation{\instPanjab} % 5163
  \author{M.~Barrett}\affiliation{\instKEK} % 2180
% \author{G.~Batignani}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % 6643
  \author{J.~Baudot}\affiliation{\instIPHC} % 2562
  \author{M.~Bauer}\affiliation{\instKarlsruhe} % 9863
  \author{A.~Baur}\affiliation{\instDESY} % 5683
  \author{A.~Beaubien}\affiliation{\instVictoria} % 6683
% \author{A.~Beaulieu}\affiliation{\instVictoria} % 2444
  \author{J.~Becker}\affiliation{\instKarlsruhe} % 5403
  \author{P.~K.~Behera}\affiliation{\instIITMadras} % 4204
  \author{J.~V.~Bennett}\affiliation{\instMississippi} % 2454
  \author{E.~Bernieri}\affiliation{\instRomaTreINFN} % 4483
  \author{F.~U.~Bernlochner}\affiliation{\instBonn} % 2282
  \author{V.~Bertacchi}\affiliation{\instCPPM} % 2212
  \author{M.~Bertemes}\affiliation{\instBNL} % 2595
  \author{E.~Bertholet}\affiliation{\instTelAviv} % 13163
  \author{M.~Bessner}\affiliation{\instHawaii} % 3783
  \author{S.~Bettarini}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % 2350
  \author{V.~Bhardwaj}\affiliation{\instIISER} % 2228
  \author{B.~Bhuyan}\affiliation{\instIITGuwahati} % 2097
  \author{F.~Bianchi}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2564
  \author{T.~Bilka}\affiliation{\instPrague} % 2484
  \author{S.~Bilokin}\affiliation{\instLMU} % 3623
  \author{D.~Biswas}\affiliation{\instLouisville} % 8703
% \author{A.~Bobrov}\affiliation{\instBINP}\affiliation{\instNSU} % 2294
  \author{D.~Bodrov}\affiliation{\instHSE} % 9643
  \author{A.~Bolz}\affiliation{\instDESY} % 15403
% \author{A.~Bondar}\affiliation{\instBINP}\affiliation{\instNSU} % 4643
% \author{G.~Bonvicini}\affiliation{\instWayneState} % 2095
  \author{J.~Borah}\affiliation{\instIITGuwahati} % 7083
  \author{A.~Bozek}\affiliation{\instKrakow} % 2303
  \author{M.~Bra\v{c}ko}\affiliation{\instLjubljanaUM}\affiliation{\instLjubljanaJSI} % 2425
  \author{P.~Branchini}\affiliation{\instRomaTreINFN} % 2577
% \author{N.~Braun}\affiliation{\instKarlsruhe} % 2436
  \author{R.~A.~Briere}\affiliation{\instCMU} % 2584
  \author{T.~E.~Browder}\affiliation{\instHawaii} % 2560
% \author{D.~N.~Brown}\affiliation{\instLouisville} % 8743
  \author{A.~Budano}\affiliation{\instRomaTreINFN} % 2171
% \author{L.~Burmistrov}\affiliation{\instIJCLab} % 2111
  \author{S.~Bussino}\affiliation{\instRomaTreUNIV}\affiliation{\instRomaTreINFN} % 5384
  \author{M.~Campajola}\affiliation{\instNapoliINFN} % 5223
  \author{L.~Cao}\affiliation{\instDESY} % 2099
  \author{G.~Casarosa}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % 2491
  \author{C.~Cecchi}\affiliation{\instPerugiaINFN}\affiliation{\instPerugiaUNIV} % 2433
% \author{J.~Cerasoli}\affiliation{\instIPHC} % 20746
% \author{D.~\v{C}ervenkov}\affiliation{\instPrague} % 2078
  \author{M.-C.~Chang}\affiliation{\instFuJen} % 2827
  \author{P.~Chang}\affiliation{\instNTUTaiwan} % 2542
  \author{R.~Cheaib}\affiliation{\instDESY} % 2208
  \author{P.~Cheema}\affiliation{\instSydney} % 15264
  \author{V.~Chekelian}\affiliation{\instMPP} % 2167
  \author{C.~Chen}\affiliation{\instISU} % 12803
% \author{Y.~Q.~Chen}\affiliation{\instUSTC} % 2576
  \author{Y.~Q.~Chen}\affiliation{\instHUNNU} % 16264
% \author{Y.-T.~Chen}\affiliation{\instNTUTaiwan} % 2884
  \author{B.~G.~Cheon}\affiliation{\instHanyang} % 2173
  \author{K.~Chilikin}\affiliation{\instBINP} % 2308
  \author{K.~Chirapatpimol}\affiliation{\instChiangMai} % 10803
  \author{H.-E.~Cho}\affiliation{\instHanyang} % 2182
  \author{K.~Cho}\affiliation{\instKISTI} % 2516
  \author{S.-J.~Cho}\affiliation{\instYonsei} % 2723
  \author{S.-K.~Choi}\affiliation{\instCAU} % 2364
  \author{S.~Choudhury}\affiliation{\instISU} % 2206
  \author{D.~Cinabro}\affiliation{\instWayneState} % 2092
  \author{J.~Cochran}\affiliation{\instISU} % 12604
  \author{L.~Corona}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % 3944
% \author{L.~M.~Cremaldi}\affiliation{\instMississippi} % 2276
  \author{S.~Cunliffe}\affiliation{\instDESY} % 2272
% \author{T.~Czank}\affiliation{\instTokyoMetropolitan} % 2254
  \author{S.~Das}\affiliation{\instMNITJaipur} % 9163
% \author{N.~Dash}\affiliation{\instIITMadras} % 2601
  \author{F.~Dattola}\affiliation{\instDESY} % 3745
  \author{E.~De~La~Cruz-Burelo}\affiliation{\instCinvestavIPN} % 2359
  \author{S.~A.~De~La~Motte}\affiliation{\instAdelaide} % 2128
  \author{G.~de~Marino}\affiliation{\instIJCLab} % 8364
  \author{G.~De~Nardo}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % 2459
  \author{M.~De~Nuccio}\affiliation{\instUBC} % 2610
  \author{G.~De~Pietro}\affiliation{\instRomaTreINFN} % 2528
  \author{R.~de~Sangro}\affiliation{\instFrascati} % 2524
% \author{B.~Deschamps}\affiliation{\instBonn} % 2671
  \author{M.~Destefanis}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2594
  \author{S.~Dey}\affiliation{\instTelAviv} % 5023
  \author{A.~De~Yta-Hernandez}\affiliation{\instCinvestavIPN} % 2104
  \author{R.~Dhamija}\affiliation{\instIITHyderabad} % 9465
  \author{A.~Di~Canto}\affiliation{\instBNL} % 10963
  \author{F.~Di~Capua}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % 2065
% \author{S.~Di~Carlo}\affiliation{\instIJCLab} % 2079
% \author{J.~Dingfelder}\affiliation{\instBonn} % 2151
  \author{Z.~Dole\v{z}al}\affiliation{\instPrague} % 2319
  \author{I.~Dom\'{\i}nguez~Jim\'{e}nez}\affiliation{\instUAS} % 2191
  \author{T.~V.~Dong}\affiliation{\instITAR} % 2215
  \author{M.~Dorigo}\affiliation{\instTriesteINFN} % 12543
  \author{K.~Dort}\affiliation{\instGiessen} % 5583
  \author{D.~Dossett}\affiliation{\instMelbourne} % 2574
  \author{S.~Dreyer}\affiliation{\instDESY} % 12823
  \author{S.~Dubey}\affiliation{\instHawaii} % 11063
% \author{S.~Duell}\affiliation{\instBonn} % 2344
  \author{G.~Dujany}\affiliation{\instIPHC} % 9703
  \author{P.~Ecker}\affiliation{\instKarlsruhe} % 5563
  \author{M.~Eliachevitch}\affiliation{\instBonn} % 2725
% \author{D.~Epifanov}\affiliation{\instBINP}\affiliation{\instNSU} % 2551
  \author{P.~Feichtinger}\affiliation{\instHEPHYVienna} % 9843
  \author{T.~Ferber}\affiliation{\instKarlsruhe} % 2482
  \author{D.~Ferlewicz}\affiliation{\instMelbourne} % 2073
  \author{T.~Fillinger}\affiliation{\instIPHC} % 9803
  \author{C.~Finck}\affiliation{\instIPHC} % 15803
  \author{G.~Finocchiaro}\affiliation{\instFrascati} % 2400
% \author{P.~Fischer}\affiliation{\instHeidelberg} % 2141
% \author{K.~Flood}\affiliation{\instHawaii} % 12103
  \author{A.~Fodor}\affiliation{\instMcGill} % 2312
  \author{F.~Forti}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % 2432
  \author{A.~Frey}\affiliation{\instGoettingen} % 2150
% \author{M.~Friedl}\affiliation{\instHEPHYVienna} % 2442
  \author{B.~G.~Fulsom}\affiliation{\instPNNL} % 2563
% \author{M.~Gabriel}\affiliation{\instMPP} % 2443
  \author{A.~Gabrielli}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 13523
% \author{N.~Gabyshev}\affiliation{\instBINP}\affiliation{\instNSU} % 2510
  \author{E.~Ganiev}\affiliation{\instDESY} % 4623
  \author{M.~Garcia-Hernandez}\affiliation{\instCinvestavIPN} % 4823
% \author{R.~Garg}\affiliation{\instPanjab} % 2213
% \author{A.~Garmash}\affiliation{\instBINP}\affiliation{\instNSU} % 2161
  \author{G.~Gaudino}\affiliation{\instNapoliINFN} % 16563
  \author{V.~Gaur}\affiliation{\instUPES} % 2413
% \author{A.~Gaz}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 2181
% \author{U.~Gebauer}\affiliation{\instGoettingen} % 2174
  \author{A.~Gellrich}\affiliation{\instDESY} % 2480
% \author{J.~Gemmler}\affiliation{\instKarlsruhe} % 2321
% \author{T.~Ge{\ss}ler}\affiliation{\instGiessen} % 2121
  \author{G.~Ghevondyan}\affiliation{\instYerevan} % 9445
% \author{G.~Giakoustidis}\affiliation{\instBonn} % 13723
  \author{R.~Giordano}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2103
  \author{A.~Giri}\affiliation{\instIITHyderabad} % 2106
% \author{A.~Glazov}\affiliation{\instDESY} % 2473
  \author{B.~Gobbo}\affiliation{\instTriesteINFN} % 2109
  \author{R.~Godang}\affiliation{\instSAlabama} % 2449
  \author{P.~Goldenzweig}\affiliation{\instKarlsruhe} % 2345
% \author{B.~Golob}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI}\affiliation{\instNovaGorica} % 3703
% \author{P.~Gomis}\affiliation{\instIFIC} % 2354
% \author{G.~Gong}\affiliation{\instUSTC} % 2727
% \author{P.~Grace}\affiliation{\instAdelaide} % 9563
  \author{W.~Gradl}\affiliation{\instMainz} % 2570
  \author{T.~Grammatico}\affiliation{\instVictoria} % 20623
  \author{S.~Granderath}\affiliation{\instBonn} % 8383
  \author{E.~Graziani}\affiliation{\instRomaTreINFN} % 2342
  \author{D.~Greenwald}\affiliation{\instTUM} % 2686
  \author{Z.~Gruberov\'{a}}\affiliation{\instPrague} % 8824
  \author{T.~Gu}\affiliation{\instPittsburgh} % 14283
  \author{Y.~Guan}\affiliation{\instCincinnati} % 2514
  \author{K.~Gudkova}\affiliation{\instBINP}\affiliation{\instNSU} % 10504
  \author{J.~Guilliams}\affiliation{\instMississippi} % 13543
% \author{C.~Hadjivasiliou}\affiliation{\instPNNL} % 9503
  \author{S.~Halder}\affiliation{\instTata} % 4743
% \author{K.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2462
  \author{T.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2523
% \author{O.~Hartbrich}\affiliation{\instHawaii} % 2158
  \author{K.~Hayasaka}\affiliation{\instNiigata} % 2330
  \author{H.~Hayashii}\affiliation{\instNaraWu} % 2455
  \author{S.~Hazra}\affiliation{\instTata} % 7663
  \author{C.~Hearty}\affiliation{\instUBC}\affiliation{\instIPP} % 2450
  \author{M.~T.~Hedges}\affiliation{\instBonn} % 2265
  \author{I.~Heredia~de~la~Cruz}\affiliation{\instCinvestavIPN}\affiliation{\instConacyt} % 2559
  \author{M.~Hern\'{a}ndez~Villanueva}\affiliation{\instDESY} % 2466
  \author{A.~Hershenhorn}\affiliation{\instUBC} % 2552
  \author{T.~Higuchi}\affiliation{\instIPMU} % 2485
  \author{E.~C.~Hill}\affiliation{\instUBC} % 7823
% \author{H.~Hirata}\affiliation{\instNagoya} % 2070
% \author{M.~Hoek}\affiliation{\instMainz} % 2101
  \author{M.~Hohmann}\affiliation{\instMelbourne} % 2077
% \author{S.~Hollitt}\affiliation{\instAdelaide} % 2557
% \author{T.~Hotta}\affiliation{\instRCNP} % 2084
  \author{C.-L.~Hsu}\affiliation{\instSydney} % 2299
% \author{K.~Huang}\affiliation{\instNTUTaiwan} % 2389
  \author{T.~Humair}\affiliation{\instMPP} % 10643
  \author{T.~Iijima}\affiliation{\instNagoya}\affiliation{\instKEK}\affiliation{\instNagoyaKMI} % 2446
  \author{K.~Inami}\affiliation{\instNagoya}\affiliation{\instKEK} % 2323
  \author{G.~Inguglia}\affiliation{\instHEPHYVienna} % 2500
  \author{N.~Ipsita}\affiliation{\instIITHyderabad} % 12223
% \author{J.~Irakkathil~Jabbar}\affiliation{\instKarlsruhe} % 7343
  \author{A.~Ishikawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2281
  \author{S.~Ito}\affiliation{\instKEK} % 17463
  \author{R.~Itoh}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2487
  \author{M.~Iwasaki}\affiliation{\instOsakaMetropolitan} % 2360
% \author{Y.~Iwasaki}\affiliation{\instKEK} % 2229
% \author{S.~Iwata}\affiliation{\instTokyoMetropolitan} % 4323
  \author{P.~Jackson}\affiliation{\instAdelaide} % 2255
  \author{W.~W.~Jacobs}\affiliation{\instIndiana} % 2322
  \author{D.~E.~Jaffe}\affiliation{\instBNL} % 3663
  \author{E.-J.~Jang}\affiliation{\instGyeongsang} % 6744
% \author{M.~Jeandron}\affiliation{\instMississippi} % 2806
% \author{H.~B.~Jeon}\affiliation{\instKyungpook} % 2170
  \author{Q.~P.~Ji}\affiliation{\instHNU} % 16243
  \author{S.~Jia}\affiliation{\instFudan} % 2457
  \author{Y.~Jin}\affiliation{\instTriesteINFN} % 2105
% \author{C.~Joo}\affiliation{\instIPMU} % 3525
  \author{K.~K.~Joo}\affiliation{\instChonnam} % 4224
  \author{H.~Junkerkalefeld}\affiliation{\instBonn} % 12963
% \author{I.~Kadenko}\affiliation{\instKyiv} % 3843
% \author{J.~Kahn}\affiliation{\instKarlsruhe} % 2448
  \author{H.~Kakuno}\affiliation{\instTokyoMetropolitan} % 2391
  \author{M.~Kaleta}\affiliation{\instKrakow} % 5603
% \author{D.~Kalita}\affiliation{\instIITGuwahati} % 2220
  \author{A.~B.~Kaliyar}\affiliation{\instHEPHYVienna} % 7344
  \author{J.~Kandra}\affiliation{\instPrague} % 2541
  \author{K.~H.~Kang}\affiliation{\instIPMU} % 2283
  \author{S.~Kang}\affiliation{\instISU} % 12683
% \author{P.~Kapusta}\affiliation{\instKrakow} % 6663
  \author{R.~Karl}\affiliation{\instDESY} % 10923
% \author{G.~Karyan}\affiliation{\instYerevan} % 2550
% \author{Y.~Kato}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2549
% \author{H.~Kawai}\affiliation{\instChiba} % 4344
  \author{T.~Kawasaki}\affiliation{\instKitasato} % 4363
% \author{C.~Ketter}\affiliation{\instHawaii} % 2236
% \author{H.~Kichimi}\affiliation{\instKEK} % 2233
  \author{C.~Kiesling}\affiliation{\instMPP} % 2168
  \author{C.-H.~Kim}\affiliation{\instHanyang} % 2358
  \author{D.~Y.~Kim}\affiliation{\instSoongsil} % 2315
% \author{H.~J.~Kim}\affiliation{\instKyungpook} % 4863
  \author{K.-H.~Kim}\affiliation{\instKISTI} % 2118
% \author{K.~Kim}\affiliation{\instKoreaUnivKU} % 2409
% \author{S.-H.~Kim}\affiliation{\instSeoul} % 2428
  \author{Y.-K.~Kim}\affiliation{\instYonsei} % 2379
% \author{Y.~J.~Kim}\affiliation{\instKoreaUnivKU} % 2403
% \author{T.~D.~Kimmel}\affiliation{\instVPI} % 2241
  \author{H.~Kindo}\affiliation{\instVPI}\affiliation{\instKEK} % 2195
  \author{K.~Kinoshita}\affiliation{\instCincinnati} % 2318
% \author{C.~Kleinwort}\affiliation{\instDESY} % 2499
% \author{B.~Knysh}\affiliation{\instIJCLab} % 8883
  \author{P.~Kody\v{s}}\affiliation{\instPrague} % 2407
  \author{T.~Koga}\affiliation{\instKEK} % 6963
  \author{S.~Kohani}\affiliation{\instHawaii} % 9143
  \author{K.~Kojima}\affiliation{\instNagoya} % 6363
% \author{I.~Komarov}\affiliation{\instDESY} % 2210
  \author{T.~Konno}\affiliation{\instKitasato} % 2490
  \author{A.~Korobov}\affiliation{\instBINP}\affiliation{\instNSU} % 4185
  \author{S.~Korpar}\affiliation{\instLjubljanaUM}\affiliation{\instLjubljanaJSI} % 2475
% \author{E.~Kou}\affiliation{\instIJCLab} % 3765
% \author{N.~Kovalchuk}\affiliation{\instDESY} % 6964
  \author{E.~Kovalenko}\affiliation{\instBINP}\affiliation{\instNSU} % 3884
  \author{R.~Kowalewski}\affiliation{\instVictoria} % 2293
  \author{T.~M.~G.~Kraetzschmar}\affiliation{\instMPP} % 7543
% \author{F.~Krinner}\affiliation{\instMPP} % 9383
  \author{P.~Kri\v{z}an}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2474
% \author{R.~Kroeger}\affiliation{\instMississippi} % 2242
% \author{J.~F.~Krohn}\affiliation{\instMelbourne} % 2502
  \author{P.~Krokovny}\affiliation{\instBINP}\affiliation{\instNSU} % 2575
% \author{H.~Kr\"uger}\affiliation{\instBonn} % 2290
% \author{W.~Kuehn}\affiliation{\instGiessen} % 2534
  \author{T.~Kuhr}\affiliation{\instLMU} % 2486
  \author{J.~Kumar}\affiliation{\instCMU} % 6464
% \author{M.~Kumar}\affiliation{\instIISER} % 2744
  \author{R.~Kumar}\affiliation{\instPanjabPAU} % 2189
  \author{K.~Kumara}\affiliation{\instMississippi} % 2257
% \author{T.~Kumita}\affiliation{\instTokyoMetropolitan} % 4083
  \author{T.~Kunigo}\affiliation{\instKEK} % 10104
% \author{M.~K\"{u}nzel}\affiliation{\instDESY}\affiliation{\instLMU} % 2139
% \author{S.~Kurz}\affiliation{\instDESY} % 9363
  \author{A.~Kuzmin}\affiliation{\instBINP}\affiliation{\instNSU} % 2520
% \author{P.~Kvasni\v{c}ka}\affiliation{\instPrague} % 2184
  \author{Y.-J.~Kwon}\affiliation{\instYonsei} % 2231
  \author{S.~Lacaprara}\affiliation{\instPadovaINFN} % 2447
% \author{Y.-T.~Lai}\affiliation{\instIPMU} % 2066
% \author{C.~La~Licata}\affiliation{\instIPMU} % 2348
% \author{K.~Lalwani}\affiliation{\instMNITJaipur} % 2142
  \author{T.~Lam}\affiliation{\instVPI} % 2729
  \author{L.~Lanceri}\affiliation{\instTriesteINFN} % 2540
  \author{J.~S.~Lange}\affiliation{\instGiessen} % 2277
  \author{M.~Laurenza}\affiliation{\instRomaTreINFN}\affiliation{\instRomaTreUNIV} % 10223
  \author{K.~Lautenbach}\affiliation{\instCPPM} % 2102
% \author{P.~J.~Laycock}\affiliation{\instBNL} % 7683
  \author{R.~Leboucher}\affiliation{\instCPPM} % 14083
  \author{F.~R.~Le~Diberder}\affiliation{\instIJCLab} % 3267
% \author{I.-S.~Lee}\affiliation{\instHanyang} % 2422
% \author{S.~C.~Lee}\affiliation{\instKyungpook} % 2544
  \author{P.~Leitl}\affiliation{\instMPP} % 2414
% \author{D.~Levit}\affiliation{\instKEK} % 2507
% \author{P.~M.~Lewis}\affiliation{\instBonn} % 2582
  \author{C.~Li}\affiliation{\instLNNU} % 2325
  \author{L.~K.~Li}\affiliation{\instCincinnati} % 3263
% \author{S.~X.~Li}\affiliation{\instFudan} % 2377
  \author{Y.~B.~Li}\affiliation{\instFudan} % 2573
  \author{J.~Libby}\affiliation{\instIITMadras} % 2262
  \author{K.~Lieret}\affiliation{\instLMU} % 2268
% \author{J.~Lin}\affiliation{\instNTUTaiwan} % 2401
  \author{Z.~Liptak}\affiliation{\instHiroshima} % 3565
  \author{Q.~Y.~Liu}\affiliation{\instDESY} % 7045
% \author{Z.~A.~Liu}\affiliation{\instIHEPChina} % 3283
  \author{Z.~Q.~Liu}\affiliation{\instShandong} % 11303
  \author{D.~Liventsev}\affiliation{\instWayneState}\affiliation{\instKEK} % 2578
  \author{S.~Longo}\affiliation{\instDESY} % 2396
% \author{A.~Loos}\affiliation{\instSCarolina} % 2356
  \author{A.~Lozar}\affiliation{\instLjubljanaJSI} % 12423
% \author{P.~Lu}\affiliation{\instNTUTaiwan} % 2148
  \author{T.~Lueck}\affiliation{\instLMU} % 2406
% \author{F.~Luetticke}\affiliation{\instBonn} % 2533
% \author{T.~Luo}\affiliation{\instFudan} % 3268
  \author{C.~Lyu}\affiliation{\instBonn} % 12484
% \author{Y.~Ma}\affiliation{\instRIKENMSL} % 16883
  \author{M.~Maggiora}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 5343
  \author{S.~P.~Maharana}\affiliation{\instIITHyderabad} % 19083
  \author{R.~Maiti}\affiliation{\instHEPHYVienna} % 12043
  \author{S.~Maity}\affiliation{\instIITBhubaneswar} % 2985
  \author{R.~Manfredi}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 10303
  \author{E.~Manoni}\affiliation{\instPerugiaINFN} % 2305
  \author{A.~C.~Manthei}\affiliation{\instBonn} % 15023
  \author{M.~Mantovano}\affiliation{\instTriesteINFN}\affiliation{\instTriesteUNIV} % 19783
% \author{D.~Marcantonio}\affiliation{\instMelbourne} % 11163
  \author{S.~Marcello}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 4223
  \author{C.~Marinas}\affiliation{\instIFIC} % 2133
  \author{L.~Martel}\affiliation{\instIPHC} % 13503
  \author{C.~Martellini}\affiliation{\instRomaTreINFN} % 16983
  \author{A.~Martini}\affiliation{\instDESY} % 2336
  \author{T.~Martinov}\affiliation{\instDESY} % 19463
  \author{L.~Massaccesi}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 16323
% \author{M.~Masuda}\affiliation{\instRCNP}\affiliation{\instEri} % 2238
  \author{T.~Matsuda}\affiliation{\instUOM} % 5543
  \author{K.~Matsuoka}\affiliation{\instKEK}\affiliation{\instNagoya} % 2316
  \author{D.~Matvienko}\affiliation{\instBINP}\affiliation{\instNSU} % 2351
  \author{S.~K.~Maurya}\affiliation{\instIITGuwahati} % 9763
  \author{J.~A.~McKenna}\affiliation{\instUBC} % 2392
% \author{J.~McNeil}\affiliation{\instFlorida} % 2382
% \author{F.~Meggendorfer}\affiliation{\instMPP} % 7103
  \author{F.~Meier}\affiliation{\instDuke} % 3103
  \author{M.~Merola}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % 2456
  \author{F.~Metzner}\affiliation{\instKarlsruhe} % 2296
  \author{M.~Milesi}\affiliation{\instMelbourne} % 5443
  \author{C.~Miller}\affiliation{\instVictoria} % 2273
  \author{K.~Miyabayashi}\affiliation{\instNaraWu}\affiliation{\instKEK} % 2327
  \author{H.~Miyake}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2452
% \author{H.~Miyata}\affiliation{\instNiigata} % 2071
  \author{R.~Mizuk}\affiliation{\instHSE} % 2483
% \author{K.~Azmi}\affiliation{\instMalaya} % 2506
  \author{G.~B.~Mohanty}\affiliation{\instTata} % 2278
  \author{N.~Molina-Gonzalez}\affiliation{\instCinvestavIPN} % 8004
  \author{S.~Moneta}\affiliation{\instPerugiaUNIV}\affiliation{\instPerugiaINFN} % 13303
% \author{H.~Moon}\affiliation{\instKoreaUnivKU} % 2304
% \author{T.~Moon}\affiliation{\instSeoul} % 2397
% \author{J.~A.~Mora~Grimaldo}\affiliation{\instUTokyo} % 4403
% \author{T.~Morii}\affiliation{\instIPMU} % 3543
  \author{H.-G.~Moser}\affiliation{\instMPP} % 2120
  \author{M.~Mrvar}\affiliation{\instHEPHYVienna} % 2527
% \author{F.~J.~M\"{u}ller}\affiliation{\instDESY} % 2123
% \author{Th.~Muller}\affiliation{\instKarlsruhe} % 2165
% \author{G.~Muroyama}\affiliation{\instNagoya} % 2093
% \author{C.~Murphy}\affiliation{\instIPMU} % 12403
  \author{R.~Mussa}\affiliation{\instTorinoINFN} % 2372
  \author{I.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 3463
  \author{K.~R.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2417
% \author{E.~Nakano}\affiliation{\instOsakaMetropolitan} % 2554
  \author{M.~Nakao}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2498
  \author{H.~Nakayama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2232
% \author{H.~Nakazawa}\affiliation{\instNTUTaiwan} % 2335
  \author{Y.~Nakazawa}\affiliation{\instKEK} % 17383
  \author{A.~Narimani~Charan}\affiliation{\instDESY} % 10143
  \author{M.~Naruki}\affiliation{\instKyotoU} % 4583
  \author{D.~Narwal}\affiliation{\instIITGuwahati} % 7223
  \author{Z.~Natkaniec}\affiliation{\instKrakow} % 3923
  \author{A.~Natochii}\affiliation{\instHawaii} % 12063
  \author{L.~Nayak}\affiliation{\instIITHyderabad} % 9464
  \author{M.~Nayak}\affiliation{\instTelAviv} % 2371
  \author{G.~Nazaryan}\affiliation{\instYerevan} % 9523
% \author{D.~Neverov}\affiliation{\instNagoya} % 2075
  \author{C.~Niebuhr}\affiliation{\instDESY} % 2477
% \author{M.~Niiyama}\affiliation{\instKSU} % 2063
% \author{J.~Ninkovic}\affiliation{\instMPGHLL} % 2386
  \author{N.~K.~Nisar}\affiliation{\instBNL} % 2522
  \author{S.~Nishida}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2571
% \author{K.~Nishimura}\affiliation{\instHawaii} % 3063
% \author{M.~H.~A.~Nouxman}\affiliation{\instMalaya} % 2470
% \author{K.~Ogawa}\affiliation{\instNiigata} % 2430
  \author{S.~Ogawa}\affiliation{\instToho} % 6263
% \author{S.~L.~Olsen}\affiliation{\instCAU} % 4563
% \author{Y.~Onishchuk}\affiliation{\instKyiv} % 2157
  \author{H.~Ono}\affiliation{\instNiigata} % 2160
  \author{Y.~Onuki}\affiliation{\instUTokyo} % 2331
  \author{P.~Oskin}\affiliation{\instIJCLab} % 9623
% \author{F.~Otani}\affiliation{\instUTokyo} % 16244
% \author{E.~R.~Oxford}\affiliation{\instCMU} % 6943
% \author{H.~Ozaki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2984
  \author{P.~Pakhlov}\affiliation{\instHSE} % 2221
  \author{G.~Pakhlova}\affiliation{\instHSE} % 2188
  \author{A.~Paladino}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % 2435
% \author{T.~Pang}\affiliation{\instPittsburgh} % 2114
  \author{A.~Panta}\affiliation{\instMississippi} % 7943
  \author{E.~Paoloni}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % 2488
  \author{S.~Pardi}\affiliation{\instNapoliINFN} % 2532
  \author{K.~Parham}\affiliation{\instDuke} % 10684
  \author{H.~Park}\affiliation{\instKyungpook} % 2284
  \author{J.~Park}\affiliation{\instYonsei} % 18203
  \author{S.-H.~Park}\affiliation{\instKEK} % 2509
  \author{B.~Paschen}\affiliation{\instBonn} % 2159
  \author{A.~Passeri}\affiliation{\instRomaTreINFN} % 2116
% \author{A.~Pathak}\affiliation{\instLouisville} % 8723
  \author{S.~Patra}\affiliation{\instIISER} % 3123
  \author{S.~Paul}\affiliation{\instTUM} % 2131
  \author{T.~K.~Pedlar}\affiliation{\instLuther} % 2421
  \author{I.~Peruzzi}\affiliation{\instFrascati} % 2253
  \author{R.~Peschke}\affiliation{\instHawaii} % 7123
  \author{R.~Pestotnik}\affiliation{\instLjubljanaJSI} % 2476
  \author{F.~Pham}\affiliation{\instMelbourne} % 2963
  \author{M.~Piccolo}\affiliation{\instFrascati} % 2147
  \author{L.~E.~Piilonen}\affiliation{\instVPI} % 2346
  \author{G.~Pinna~Angioni}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 13363
  \author{P.~L.~M.~Podesta-Lerma}\affiliation{\instUAS} % 2266
  \author{T.~Podobnik}\affiliation{\instLjubljanaJSI} % 11223
  \author{S.~Pokharel}\affiliation{\instMississippi} % 12283
  \author{L.~Polat}\affiliation{\instCPPM} % 9783
% \author{V.~Popov}\affiliation{\instHSE} % 2096
  \author{C.~Praz}\affiliation{\instDESY} % 2726
  \author{S.~Prell}\affiliation{\instISU} % 12743
  \author{E.~Prencipe}\affiliation{\instGiessen} % 2219
  \author{M.~T.~Prim}\affiliation{\instBonn} % 2501
% \author{M.~V.~Purohit}\affiliation{\instOkinawa} % 2196
  \author{H.~Purwar}\affiliation{\instHawaii} % 12363
  \author{N.~Rad}\affiliation{\instDESY} % 11683
  \author{P.~Rados}\affiliation{\instHEPHYVienna} % 7383
  \author{G.~Raeuber}\affiliation{\instHEPHYVienna} % 18143
  \author{S.~Raiz}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 13003
  \author{A.~Ramirez~Morales}\affiliation{\instKyungpook} % 13724
% \author{R.~Rasheed}\affiliation{\instIPHC} % 3643
% \author{N.~Rauls}\affiliation{\instGoettingen} % 11603
  \author{M.~Reif}\affiliation{\instMPP} % 8043
  \author{S.~Reiter}\affiliation{\instGiessen} % 2248
  \author{M.~Remnev}\affiliation{\instBINP}\affiliation{\instNSU} % 2785
  \author{I.~Ripp-Baudot}\affiliation{\instIPHC} % 2469
% \author{M.~Ritter}\affiliation{\instLMU} % 2580
% \author{M.~Ritzert}\affiliation{\instHeidelberg} % 2526
  \author{G.~Rizzo}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % 2579
  \author{L.~B.~Rizzuto}\affiliation{\instLjubljanaJSI} % 3746
  \author{S.~H.~Robertson}\affiliation{\instMcGill}\affiliation{\instIPP} % 2471
% \author{P.~Rocchetti}\affiliation{\instMelbourne} % 13763
  \author{D.~Rodr\'{i}guez~P\'{e}rez}\affiliation{\instUAS} % 2176
% \author{M.~Roehrken}\affiliation{\instDESY} % 11883
  \author{J.~M.~Roney}\affiliation{\instVictoria}\affiliation{\instIPP} % 2244
% \author{C.~Rosenfeld}\affiliation{\instSCarolina} % 2082
  \author{A.~Rostomyan}\affiliation{\instDESY} % 2481
  \author{N.~Rout}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 2965
% \author{M.~Rozanska}\affiliation{\instKrakow} % 2205
  \author{G.~Russo}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2388
% \author{D.~Sahoo}\affiliation{\instISU} % 2110
% \author{Y.~Sakai}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2175
  \author{D.~A.~Sanders}\affiliation{\instMississippi} % 2458
  \author{S.~Sandilya}\affiliation{\instIITHyderabad} % 2286
  \author{A.~Sangal}\affiliation{\instCincinnati} % 2384
  \author{L.~Santelj}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2185
% \author{P.~Sartori}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 4523
  \author{Y.~Sato}\affiliation{\instKEK} % 5243
  \author{V.~Savinov}\affiliation{\instPittsburgh} % 2292
  \author{B.~Scavino}\affiliation{\instMainz} % 2518
% \author{J.~Schmitz}\affiliation{\instBonn} % 12863
% \author{M.~Schnepf}\affiliation{\instKarlsruhe} % 15683
% \author{M.~Schram}\affiliation{\instPNNL} % 2306
% \author{H.~Schreeck}\affiliation{\instGoettingen} % 2434
  \author{J.~Schueler}\affiliation{\instHawaii} % 2824
  \author{C.~Schwanda}\affiliation{\instHEPHYVienna} % 2108
  \author{A.~J.~Schwartz}\affiliation{\instCincinnati} % 2162
% \author{B.~Schwenker}\affiliation{\instGoettingen} % 2405
% \author{M.~Schwickardi}\affiliation{\instGoettingen} % 14743
  \author{Y.~Seino}\affiliation{\instNiigata} % 2517
  \author{A.~Selce}\affiliation{\instRomaTreINFN}\affiliation{\instRomaENEA} % 9043
  \author{K.~Senyo}\affiliation{\instYamagata} % 2987
% \author{I.~S.~Seong}\affiliation{\instHawaii} % 2572
  \author{J.~Serrano}\affiliation{\instCPPM} % 12124
  \author{M.~E.~Sevior}\affiliation{\instMelbourne} % 2328
  \author{C.~Sfienti}\affiliation{\instMainz} % 2214
% \author{W.~Shan}\affiliation{\instHUNNU} % 11943
  \author{C.~Sharma}\affiliation{\instMNITJaipur} % 11584
% \author{V.~Shebalin}\affiliation{\instHawaii} % 2339
  \author{C.~P.~Shen}\affiliation{\instFudan} % 2464
  \author{X.~D.~Shi}\affiliation{\instKEK} % 18843
% \author{H.~Shibuya}\affiliation{\instToho} % 2234
  \author{T.~Shillington}\affiliation{\instMcGill} % 7983
% \author{T.~Shimasaki}\affiliation{\instUTokyo} % 16263
  \author{J.-G.~Shiu}\affiliation{\instNTUTaiwan} % 2412
% \author{D.~Shtol}\affiliation{\instBINP}\affiliation{\instNSU} % 9223
  \author{B.~Shwartz}\affiliation{\instBINP}\affiliation{\instNSU} % 2122
  \author{A.~Sibidanov}\affiliation{\instHawaii} % 2419
  \author{F.~Simon}\affiliation{\instMPP} % 2164
  \author{J.~B.~Singh}\affiliation{\instPanjab} % 2903
% \author{S.~Skambraks}\affiliation{\instKarlsruhe} % 2394
  \author{J.~Skorupa}\affiliation{\instMPP} % 12523
% \author{K.~Smith}\affiliation{\instMelbourne} % 2243
  \author{R.~J.~Sobie}\affiliation{\instVictoria}\affiliation{\instIPP} % 2472
  \author{A.~Soffer}\affiliation{\instTelAviv} % 2217
  \author{A.~Sokolov}\affiliation{\instIHEPRussia} % 2521
% \author{Y.~Soloviev}\affiliation{\instDESY} % 2479
  \author{E.~Solovieva}\affiliation{\instBINP} % 2398
  \author{S.~Spataro}\affiliation{\instTorinoINFN}\affiliation{\instTorinoUNIV} % 2117
  \author{B.~Spruck}\affiliation{\instMainz} % 2493
  \author{M.~Stari\v{c}}\affiliation{\instLjubljanaJSI} % 2326
  \author{S.~Stefkova}\affiliation{\instKarlsruhe} % 8783
  \author{Z.~S.~Stottler}\affiliation{\instVPI} % 2267
  \author{R.~Stroili}\affiliation{\instPadovaINFN}\affiliation{\instPadovaUNIV} % 2465
  \author{J.~Strube}\affiliation{\instPNNL} % 2451
% \author{J.~Stypula}\affiliation{\instKrakow} % 2368
  \author{Y.~Sue}\affiliation{\instNagoya} % 2085
% \author{R.~Sugiura}\affiliation{\instUTokyo} % 4644
  \author{M.~Sumihama}\affiliation{\instRCNP}\affiliation{\instGifu} % 4243
  \author{K.~Sumisawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2583
% \author{T.~Sumiyoshi}\affiliation{\instTokyoMetropolitan} % 4184
  \author{W.~Sutcliffe}\affiliation{\instBonn} % 3784
  \author{S.~Y.~Suzuki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2496
  \author{H.~Svidras}\affiliation{\instDESY} % 11783
% \author{M.~Tabata}\affiliation{\instChiba} % 2986
% \author{M.~Takahashi}\affiliation{\instDESY} % 2467
  \author{M.~Takizawa}\affiliation{\instSPU}\affiliation{\instJPARC}\affiliation{\instRIKENMSL} % 2437
  \author{U.~Tamponi}\affiliation{\instTorinoINFN} % 2366
% \author{S.~Tanaka}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2530
  \author{K.~Tanida}\affiliation{\instJAEA} % 3803
  \author{H.~Tanigawa}\affiliation{\instUTokyo} % 2237
% \author{N.~Taniguchi}\affiliation{\instKEK} % 2285
% \author{Y.~Tao}\affiliation{\instFlorida} % 2362
% \author{P.~Taras}\affiliation{\instMontreal} % 2202
  \author{F.~Tenchini}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2546
  \author{A.~Thaller}\affiliation{\instCPPM} % 16044
  \author{R.~Tiwary}\affiliation{\instTata} % 10403
  \author{D.~Tonelli}\affiliation{\instTriesteINFN} % 4564
  \author{E.~Torassa}\affiliation{\instPadovaINFN} % 2556
  \author{N.~Toutounji}\affiliation{\instSydney} % 2263
  \author{K.~Trabelsi}\affiliation{\instIJCLab} % 2369
  \author{I.~Tsaklidis}\affiliation{\instBonn} % 13443
% \author{T.~Tsuboyama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2361
% \author{N.~Tsuzuki}\affiliation{\instNagoya} % 2352
  \author{M.~Uchida}\affiliation{\instTitech} % 2370
  \author{I.~Ueda}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2519
% \author{S.~Uehara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2586
  \author{Y.~Uematsu}\affiliation{\instUTokyo} % 5883
% \author{T.~Ueno}\affiliation{\instTohoku} % 4364
  \author{T.~Uglov}\affiliation{\instHSE} % 2252
  \author{K.~Unger}\affiliation{\instKarlsruhe} % 9463
  \author{Y.~Unno}\affiliation{\instHanyang} % 2420
  \author{K.~Uno}\affiliation{\instNiigata} % 14963
  \author{S.~Uno}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2149
  \author{P.~Urquijo}\affiliation{\instMelbourne} % 2302
  \author{Y.~Ushiroda}\affiliation{\instKEK}\affiliation{\instUTokyo}\affiliation{\instSOKENDAI} % 2317
% \author{Y.~V.~Usov}\affiliation{\instBINP}\affiliation{\instNSU} % 5003
  \author{S.~E.~Vahsen}\affiliation{\instHawaii} % 2251
  \author{R.~van~Tonder}\affiliation{\instMcGill} % 2706
  \author{G.~S.~Varner}\affiliation{\instHawaii} % 2119
  \author{K.~E.~Varvell}\affiliation{\instSydney} % 2545
  \author{A.~Vinokurova}\affiliation{\instBINP}\affiliation{\instNSU} % 2289
  \author{V.~S.~Vismaya}\affiliation{\instIITHyderabad} % 16063
  \author{L.~Vitale}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 2415
  \author{V.~Vobbilisetti}\affiliation{\instIJCLab} % 7364
% \author{V.~Vorobyev}\affiliation{\instBINP} % 2298
  \author{A.~Vossen}\affiliation{\instDuke} % 2249
% \author{B.~Wach}\affiliation{\instMPP} % 8203
% \author{E.~Waheed}\affiliation{\instKEK} % 2226
  \author{H.~M.~Wakeling}\affiliation{\instMcGill} % 3664
  \author{S.~Wallner}\affiliation{\instMPP} % 20363
% \author{K.~Wan}\affiliation{\instUTokyo} % 2591
% \author{W.~Wan~Abdullah}\affiliation{\instMalaya} % 2280
% \author{B.~Wang}\affiliation{\instMPP} % 2569
% \author{C.~H.~Wang}\affiliation{\instNUUTaiwan} % 2224
  \author{E.~Wang}\affiliation{\instPittsburgh} % 10983
  \author{M.-Z.~Wang}\affiliation{\instNTUTaiwan} % 2074
  \author{X.~L.~Wang}\affiliation{\instFudan} % 2076
  \author{A.~Warburton}\affiliation{\instMcGill} % 2347
  \author{M.~Watanabe}\affiliation{\instNiigata} % 2309
  \author{S.~Watanuki}\affiliation{\instYonsei} % 6843
% \author{J.~Webb}\affiliation{\instMelbourne} % 2423
% \author{S.~Wehle}\affiliation{\instDESY} % 2489
  \author{M.~Welsch}\affiliation{\instBonn} % 7023
% \author{O.~Werbycka}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 6123
  \author{C.~Wessel}\affiliation{\instBonn} % 2100
  \author{J.~Wiechczynski}\affiliation{\instKrakow} % 2604
% \author{P.~Wieduwilt}\affiliation{\instGoettingen} % 2343
% \author{H.~Windel}\affiliation{\instMPP} % 2081
  \author{E.~Won}\affiliation{\instKoreaUnivKU} % 2410
% \author{L.~J.~Wu}\affiliation{\instIHEPChina} % 2704
% \author{Y.~Xie}\affiliation{\instShandong} % 20383
  \author{X.~P.~Xu}\affiliation{\instSoochow} % 4923
  \author{B.~D.~Yabsley}\affiliation{\instSydney} % 3645
  \author{S.~Yamada}\affiliation{\instKEK} % 2492
  \author{W.~Yan}\affiliation{\instUSTC} % 2094
  \author{S.~B.~Yang}\affiliation{\instKoreaUnivKU} % 2374
  \author{H.~Ye}\affiliation{\instDESY} % 2537
  \author{J.~Yelton}\affiliation{\instFlorida} % 2067
  \author{J.~H.~Yin}\affiliation{\instKoreaUnivKU} % 2365
% \author{M.~Yonenaga}\affiliation{\instTokyoMetropolitan} % 2411
  \author{Y.~M.~Yook}\affiliation{\instIHEPChina} % 2453
  \author{K.~Yoshihara}\affiliation{\instNagoya} % 12663
% \author{T.~Yoshinobu}\affiliation{\instNiigata} % 2429
  \author{C.~Z.~Yuan}\affiliation{\instIHEPChina} % 2088
  \author{Y.~Yusa}\affiliation{\instNiigata} % 2357
  \author{L.~Zani}\affiliation{\instCPPM} % 2529
  \author{Y.~Zhai}\affiliation{\instISU} % 12703
% \author{J.~Z.~Zhang}\affiliation{\instIHEPChina} % 2349
% \author{Y.~Zhang}\affiliation{\instUSTC} % 2607
  \author{Y.~Zhang}\affiliation{\instFudan} % 3303
% \author{Z.~Zhang}\affiliation{\instUSTC} % 5363
  \author{V.~Zhilich}\affiliation{\instBINP}\affiliation{\instNSU} % 4703
% \author{J.~S.~Zhou}\affiliation{\instFudan} % 12463
  \author{Q.~D.~Zhou}\affiliation{\instNagoya}\affiliation{\instNagoyaIAR}\affiliation{\instNagoyaKMI} % 7323
  \author{X.~Y.~Zhou}\affiliation{\instLNNU} % 2380
  \author{V.~I.~Zhukova}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2387
% \author{V.~Zhulanov}\affiliation{\instBINP}\affiliation{\instNSU} % 4983
  \author{R.~\v{Z}leb\v{c}\'{i}k}\affiliation{\instPrague} % 13403
\collaboration{The Belle II Collaboration}



==> belle2sym.tex <==
%%%%%   Standard symbols for use in Belle II notes and papers. 
%%%%%
%%%%%	C. Hearty	21-Oct-2014		Based on babarsym.tex; authored by D. Hitlin, D. MacFarlane, P. Dauncey, and R. Waldi
%%%%%


\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% THE NAME OF THE COLLABORATION %%%%
\def\belletwo {Belle~II}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}
\def\SixS  {\Y6S}

\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter 
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second 
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}

\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    


\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}

\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}

\def\Bpipi   {\ensuremath{B^0 \to \pi^0 \pi^0}\xspace}


\def\mbc{{\ensuremath{M_{\rm bc}}}\xspace\xspace}
\def\dele{{\ensuremath{\Delta E}\xspace\xspace}}
\def\Tc{{\ensuremath{T_{c}}\xspace\xspace}}
\def\Acp{{\ensuremath{\mathcal{A}_{\it CP}}\xspace\xspace}}
\def\Scp{{\ensuremath{\mathcal{S}_{\it CP}}\xspace\xspace}}
\def\BR{{\ensuremath{\mathcal{B}}}}
\def\qr{{\ensuremath{q \cdot r}\xspace\xspace}}

